Bundle gerbes and the Weyl map

This masters thesis reviews bundle gerbe theory and the well-known basic bundle gerbe over SU(n). We introduce the cup product bundle gerbe, and show it is stably isomorphic to the pullback of the basic bundle gerbe by the Weyl map. This result enriches our understanding of the basic bundle gerbe, which has numerous applications in physics.

==> chapter3-5/CHP3.5.tex <==
%!TEX root = ../thesis.tex

	
	\chapter{Cup product bundle gerbe}
	In the proceeding example we construct the \textit{cup product} bundle gerbe, which will be central to our research. The definition of the cup product bundle gerbe is motivated by the cup product map of \v{C}ech cocycles. Given sheaves of abelian groups $F$ and $G$, the cup product
	$$\cup: C^p(\mathcal{U}, F)\otimes C^{q}(\mathcal{U}, G) \to C^{p+q}(\mathcal{U}, F\otimes G)$$ is defined by mapping  $(\underline{\alpha}, \underline{\beta})\mapsto \underline{\alpha}\cup \underline{\beta}$ where $$(\underline{\alpha}\cup \underline{\beta})_{i_0, ..., i_{p+q}} := \alpha_{i_0, ..., i_p}\otimes \beta_{i_q, ..., i_{p+q}}. $$ In particular, taking $F = \Z(1)_D$, $Q = \Z(2)_D$, $p=1$ and $q=2$, the cup product induces a map of \v{C}ech hypercohomology groups, and hence of sheaf hypercohomology groups, \begin{align}\label{eqn cup product} \cup: H^1(M, \Z(1)_D)\otimes H^{2}(M, \Z(2)_D) \to H^{3}(M, \Z(3)_D).\end{align} 
	Recall that smooth maps $f:M\to U(1)$, line bundles with connection, and bundle gerbes with connective structure are classified by $H^1(M, \Z(1)_D)$, $H^{2}(M, \Z(2)_D)$, and $H^3(M, \Z(3)_D)$ respectively (Remark \ref{remark deligne cohomology of line bundles and functions}). Therefore by Equation \ref{eqn cup product} we expect the cup product to define a bundle gerbe $(f\cup L, Y, M)$ given a map $f: M\to U(1)$ and a line bundle $L\to M$ with connection. Of course, the Deligne class of $(f\cup L, Y, M)$ will then equal the cup product of Deligne classes of $f$ and $L\to Y$.
	
	
	This construction describes how a bundle gerbe can be formed given a smooth map $M\to S^1$ and a line bundle over $M$. The set up is as follows. Let $M$ be a smooth manifold, $\pi: P\to M$ be a line bundle, and $f:M\to S^1$ be a smooth map. Let $\R\to S^1$ be the principal $\Z$-bundle with projection $x\mapsto [x]$ the quotient map by $\Z$. The given information is depicted below.% As we shall see, the map $f:M\to S^1$ allows us to construct a bundle gerbe over $M$ from a line bundle over $M$. 
	
	\begin{center} 
		\begin{tikzcd}
			P  \arrow[swap]{d}{\pi}       
			&\R \arrow{d}{[\cdot]} \\
			M  \arrow[swap]{r}{f}
			&S^1
		\end{tikzcd} 
		\text{}\\ \text{}\\ { \color{red}{Label this diagram }} 
	\end{center}
	By pulling back $\R \to S^1$ along $f$, we obtain a $\Z$-bundle $f^{-1}(\R)$ over $M$. The space $f^{-1}(\R)$ consists of pairs $(m, t) \in M\times \R$ with $f(m) = [t]$. By Example \ref{fibreproductexample} the second fibre product of $f^{-1}(\R)$ consists of triples $(m, t_1, t_2)\in M\times \R\times \R$ with $f(m) = [t_1]=[t_2]$. Let $d: f^{-1}(\R)^{[2]}\to \Z$ be the difference map $d(m, t_1, t_2) = t_1-t_2$. Let $\pi_M: f^{-1}(\R)^{[2]} \to M$ be projection. Define a line bundle $P\cup f\to f^{-1}(\R)^{[2]}$ by $$P\cup f := \pi_M^{-1}\left(P\right)^d$$ using the notation from Example \ref{powerlinebundles}. To be completely explicit, for $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$, $$(P\cup f)_{(m, t_1, t_2)} = (P_m)^{d(m,t_1, t_2)}.$$ We claim the triple $(P\cup f, f^{-1}(\R), M)$ is a bundle gerbe. The space $P\cup f$ is indeed equipped with a natural bundle gerbe multiplication. Let $(m, t_1, t_2, t_3) \in Y^{[3]}$.  Then \begin{align*}
	\pi_1^{-1}(P\cup f)\otimes \pi_3^{-1}(P\cup f)_{(m, t_1, t_2, t_3)} 
	&= (P_m)^{t_2-t_3}\otimes (P_m)^{t_1-t_2}\\
	&= (P_m)^{t_1-t_3}\\
	&= \pi_2^{-1}(P\cup f)_{(m, t_1, t_2, t_3)}. 
	\end{align*} This map is certainly a smooth isomorphism of line bundles. Associativity of the bundle gerbe multiplication  follows from associativity of the tensor product of line bundles. 
	\begin{definition}  Given a smooth manifold $M$, a smooth map $f: M\to S^1$, and a line bundle $P\to M$, the triple $(P \cup f, f^{-1}(\R), M)$ constructed above is a bundle gerbe, called the \textit{cup product bundle gerbe}. \end{definition} {\color{red}{give motivation for name by talking about DD class}} 
	\begin{center} 
		\begin{align*}
		\begin{array}{ccc}
		P \cup f      &              \\
		\downarrow &               \\
		f^{-1}(\R)^{[2]}   & \stackrel{}{\dra} f^{-1}(\R) \\
		&                   \downarrow  \\
		&                    M      \\
		\end{array}
		\end{align*}
		{\color{red}{label diagram}} 
	\end{center}
	\begin{remark}\label{isoZ}
		Note that $f^{-1}(\R)^{[2]} \cong f^{-1}(\R)\times \Z$. This follows since $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$ if $f(m) = [t_1] =[t_2]\in S^1$. The latter equality holds if and only if $t_1-t_2\in \Z$. So by identifying an element $(m, t_1, t_2)\in f^{-1}(\R)^{[2]}$ with $(m, t_1, t_1-t_2) \in  f^{-1}(\R)\times \Z$ we obtain the desired diffeomorphism. 
	\end{remark}
	\begin{example}\label{ex 1}
		In this example we look at a specific instance of the cup product bundle gerbe. We shall first define a line bundle over $T\times \su$, and will obtain from this a bundle gerbe over $T\times \su$ using the cup product construction. Let $T$ be the maximal torus of $SU(n)$ defined by $$T := \{\text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}) : \ x_1 + \cdots + x_n = 0\}\cong \left(S^1\right)^{n-1}. $$ For $i = 1, ..., n$, define the group homomorphism $$ {p}_i: T\to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n})  \mapsto e^{2\pi i x_i}.$$ For each $i=1, ..., n$, define a line bundle $\pi: {J}_i \to \frac{SU(n)}{T}$ by $${J}_i = SU(n)\times \C/\sim_{{p}_i}, $$ where $(s, z)\sim_{{p}_i} (st, {p}_i(t^{-1})z)$ for all 
		$(s, z) \in SU(n)\times U(1)$ and $t\in T$.  Denote equivalence classes in $J_i$ by $[\cdot, \cdot]_{p_i}$. It follows  that the projection $\pi: [(s, z)] \mapsto sT$ is a well-defined surjective submersion. We abuse notation and denote the pullback of $J_i$ along the projection $T\times \su \to \su$ by $J_i\to T\times \su$ throughout this work. Consider the map $$p_i: T\times\su \to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}, gT)\mapsto e^{2\pi i x_i}$$ defined for $i=1, ..., n$. 
		
		
		%	Consider the projection $$\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su\to \su$$ and define a line bundle ${J}_i \to T\times \su$ by $$J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}{J}_i'.$$
		%	%Using the constant identity-valued map $\textbf{1}_n: J_i\to T$, we can consider $J_i$ as a line bundle over $T\times \su$ with projection $1\times \pi$. 
		The elements that will be used to construct the cup product bundle gerbe are depicted below. 
		
		\begin{figure}[h!] 
			\begin{center} 
				\begin{tikzcd}
					J_i  \arrow[swap]{d}{}      
					&\R   \arrow{d}{[\cdot]}  \\
					T\times \frac{SU(n)}{T}\arrow[swap]{r}{p_i}
					&S^1
				\end{tikzcd}  \caption{Cup product bundle gerbe set up}
				\label{fig:pb1} \end{center}\end{figure} 
		%$J_{i,  {\smath{ \dfrac{SU(n)}{T} } }}, J_{i, T\times {\smath{ \dfrac{SU(n)}{T} } }}$ {\textcolor{red}{FINISH NEATENING UP NOTATION}}	Lastly, by pulling back $\R\to S^1$ by $p_i$ as before 
		Using the construction defined about, for each $i=1, ..., n$, we obtain a cup product bundle gerbe $$\left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$$ 
		%Consider the projection $$\pi_{T\times {\smath{ \dfrac{SU(n)}{T} } }}: p_i^{-1}(\R)^{[2]}\to T\times \su$$, 
		where, for any $(x_1, x_2,t,sT) \in p_i^{-1}(\R)^{[2]}$, we have $$(J_i \cup p_i)_{(x_1, x_2, t, sT)} = \left({J}_i \right)_{sT}^{x_1-x_2}.$$ %Since this fibre is independent of $t \in T$, we may sometimes abuse notation and write this fibre as $(J_i  \cup p_i)_{
		%	(x_1, x_2,sT)}$. 
		%$$(L_i\cup \varphi_i, \R^{n-1}\times  \tfrac{SU(n)}{T}, T\times  \tfrac{SU(n)}{T}). $$ {\color{red}{refer to figure}}   $$ \begin{array}{ccc}
		%L_i\cup \lambda_i         &          &        \\
		%\downarrow &         &         \\
		%\R^{n-1}\times \tfrac{SU(n)}{T}\times \Z  & \stackrel{}{\dra} &  \R^{n-1}\times \tfrac{SU(n)}{T} \\
		%&               &      \downarrow \\
		%&               &       T\times  \frac{SU(n)}{T}        \\
		%\end{array} $$
	\end{example} 
	In the following example, the product of these $n$ bundle gerbes is formed to construct a single bundle gerbe over $T\times \su$. The resulting bundle gerbe will be central to our research question. 
	\begin{remark}\label{isocup}
		%By remark \ref{isoZ}, we see that $p_i^{-1}(\R)^{[2]}\cong p_i^{-1}(\R)\times \Z$. We can also understand these spaces in terms of the original projection map $\widetilde{p}_i: T\to S^1$ as $$p_i^{-1}(\R)\cong \left(\widetilde{p}_i\right)^{-1}(\R)\times \su$$ and $$p_i^{-1}(\R)^{[2]} \cong \Z\times \left(\widetilde{p}_i\right)^{-1}(\R)\times \su.$$ 
		We can write the space $p_i^{-1}(\R)$ explicitly as $$p_i^{-1}(\R) = \left \{(t, gT, x)\in T\times \su \times \R \ \big \rvert \ t_i = [x]\right\}.$$ 
	\end{remark}
	\begin{proposition}\label{cupprodisequivariant} 
		The cup product bundle gerbes $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ defined above are $SU(n)$-equivariant for each $i=1, ..., n$. 
	\end{proposition}
	\textit{Proof}. Let us define the $SU(n)$ action on each of the spaces present in our bundle gerbe. On $T\times \su$, $SU(n)$ acts by $$g\cdot (t, hT) := (t, ghT). $$ On $p_i^{-1}(\R) = \left \{(x, t, hT) \in \R\times T\times \su \ | \ p_i(t) = [x]\right\}$, $SU(n)$ acts by $$g\cdot (x, t, hT) := (x, t, ghT), $$ and similarly for $p_i^{-1}(\R)^{[2]}$. Finally, for a standard element $\otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} \in (J_i\cup p_i)_{(x_1, x_2, hT)}$ the $SU(n)$-action is defined by $$g\cdot \otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} := \otimes_{j=1}^{x_1-x_2} [gh, v_j]_{p_i}. $$ This can be extended by linearity to define an action on any element in $J_i\cup p_i$. With these actions, $SU(n)$-equivariance of the bundle gerbe follows easily. 
	
	\begin{example}\label{exxx}
		Consider the bundle gerbes $\left(J_i \cup p_i, p_i^{-1}(\R), T\times \frac{SU(n)}{T}\right)$ for $i= 1, ..., n$ as in Example \ref{ex 1}. To describe the product of these $n$ bundle gerbes, we must first understand the fibre product $$H = p_1^{-1}(\R) \times_{T\times \frac{SU(n)}{T} }\times \cdots \times_{T\times \frac{SU(n)}{T}} p_n^{-1}(\R).$$ Since the projection from $p_i^{-1}(\R) \subseteq \R\times \left(T\times \su\right)$ to $  T\times \su$ is simply projection onto the second factor, it is clear that $$H \cong \left\{(x_1, ..., x_n, t, gT)\in \R^n \times T\times \tfrac{SU(n)}{T} \ \big\rvert\ [x_i] = p_i(t)\ \forall \  i = 1, ..., n \right\}.$$ Since the product of the diagonal entries of $t$ equals one, the condition that $[x_i] = p_i(t)$ for each $i = 1, ..., n$ can equivalently be stated as $x_1 + \cdots + x_n \in \Z$. Using this condition, and noting that $t = \text{diag}([x_1], ..., [x_n])$,  we find $$H \cong \left\{(x_1, ..., x_n, gT) \in \R^n \times \tfrac{SU(n)}{T} \ \big\rvert \ \textstyle \sum_{i=1}^n x_i \in \Z\right\}.$$ Let $W := \{(x_1, ..., x_n) \in \R^n :  \textstyle \sum_{i=1}^n x_i \in \Z\}.$ Then $H \cong W
		\times \tfrac{SU(n)}{T}.$ We remark that under this identification, the surjective submersion $H\to T\times \su$ becomes $$(x_1, ..., x_n, gT) \mapsto (\text{diag}([x_1], ..., [x_n]), gT)$$ when written as a map $W\times \su \to T\times \su$.  Therefore the tensor product from $i=1, ..., n$ of the bundle gerbes from Example \ref{ex 1} can be written as \begin{align} \label{eqn} \left(\Motimes_{i=1}^n J_i \cup p_i, W\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right). \end{align} 
	\end{example} 
	In some instances, a bundle gerbe $(P, Y, M)$ can equivalently be viewed as a bundle gerbe $(P|_{X^{[2]}}, X, M)$ for some submanifold $X\subseteq Y$. This is in fact a result of the following theorem.
	
	\begin{theorem}[\cite{stableiso}] \label{stable iso} 
		Let $\pi_1: Y\to M$, $\pi_2: X\to M$ be surjective submersions, and $f: X\to Y$ a morphism of surjective submersions, ie. $\pi_1\circ f = \pi_2$. Then a bundle gerbe $(P, Y, M)$ is stably isomorphic to $(f^{-1}(P), X, M)$. 
	\end{theorem} 
	An important consequence of this theorem occurs when $f$ is the inclusion of a submanifold into a manifold. The resulting corollary makes precise when a bundle gerbe $(P, Y, M)$ can equivalently be viewed as the bundle gerbe $(P|_{X^{[2]}}, X, M)$ for a submanifold $X\subset Y$. 
	
	
	\begin{corollary}\label{ex 2} 
		Consider a bundle gerbe $(P, Y, M)$ and a submanifold $X\subset Y$ such that $\pi|_X:X\to M$ is a surjective submersion. Let $\iota: X\to Y$ be inclusion. Then $\pi\circ \iota = \pi|_X$, therefore by Theorem \ref{stable iso} $(P, Y, M)$ is stably isomorphic to $(P|_{X^{[2]}}, X, M)$. 
	\end{corollary}
	This Corollary is most useful when the submanifold $X$ of $Y$ simplifies calculations on the bundle gerbe.  This is in fact the case for the bundle gerbe (\ref{eqn}), where the space $W \times \su$ can be replaced by the (simpler) space $\R^{n-1}\times \su$. We return to Example \ref{exxx} to make this precise. \\
	
	\noindent\textbf{Example 1.32. (Continued)} Let us justify why the space $W\times \su$ present in the bundle gerbe (\ref{eqn}) can be replaced with the space $\R^{n-1}\times \su$. First, note that $\R^{n-1}$ can be viewed as a submanifold of $W$ under the identification $$\R^{n-1} \cong \left\{(x_1, ..., x_n) \in \R^n \ \big\rvert \  \textstyle\sum_{i=1}^n x_i = 0\right\} \subseteq W.$$ Recall that the projection $W\times \su \to T\times \su$ is defined by $$ (x_1, ..., x_{n}, gT) \mapsto \left(\text{diag}\left([x_1], ...,  [x_n]\right), gT\right).$$ This map remains a surjective submersion when restricted to $\R^{n-1}\times \su$ because $T\cong (S^1)^{n-1}$. Therefore by Corollary \ref{ex 2}, the bundle gerbe (\ref{eqn}) is stably isomorphic to  $$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right) .$$
	Let us understand what this bundle gerbe looks like fibrewise. Since the projection map $\R^{n-1}\times \su \to T\times \su$ is the identity on the $\su$ factor, we have $$\left(\R^{n-1}\times \su\right)^{[2]} \cong \left(\R^{n-1}\right)^{[2]}\times \su$$ where the fibre product $\left(\R^{n-1}\right)^{[2]}$ is taken with respect to the projection $\R^{n-1}\to \left(S^1\right)^{n-1}$ given by $(x_1, ..., x_{n-1})\mapsto ([x_1], ..., [x_{n-1}])$. Let $(x, y, gT)\in \left(\R^{n-1}\right)^{[2]}\times \su$. Write $x$ and $y$ as $n$-tuples $(x_1, ..., x_n)$ and $(y_1, ..., y_n)$ respectively, whose coordinates sum to zero. Then  \begin{align}
	\left(\Motimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (J_1\cup p_1)_{(x_1, y_1, gT)} \otimes \cdots \otimes (J_n\cup p_n)_{(x_n, y_n, gT)}  \nonumber  \\
	&= (J_1)_{gT}^{d(x_1, y_1)}\otimes \cdots \otimes (J_n)_{gT}^{d(x_n, y_n)}.\label{Jifibres}
	\end{align}
	% Define for each $i=1, ..., n$ the map $p_i: \R^{n-1}\to \R$ defined by $p_i(x^1, ..., x^n)= x^i$ where again we identify $\R^{n-1}$ with the the subset of $\R^n$ whose coordinates sum to zero. Then \begin{align*}
	%\left(\bigotimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (L_1)_{gT}
	% \end{align*}
	
	The following proposition follows immediately from Propositions \ref{equivariantbundlegerbeproduct} and \ref{cupprodisequivariant}.
	\begin{proposition}
		The bundle gerbe $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ defined above is $SU(n)$-equivariant. 
	\end{proposition}
	\subsection{Geometry of the flag manifold}
	
	\indent \indent Let $F_n$ be the manifold whose points are sets $\{W_1, ..., W_n\}$ of mutually orthogonal one-dimensional subspaces of $\C^n$ ($F_n$ is the \textit{flag manifold} of $\C^n$). Let $e_1, ..., e_n$ be the standard basis vectors of $\C^n$ and define the \textit{standard element} $e$ of $F_n$ by $e := \{E_1:=\text{span}(e_1), ...,E_n:=\text{span}(e_n)\}$. Consider the action of $U(n)$ on $F_n$ defined by multiplication $$g\cdot \{W_1, ..., W_n\} := \{g W_1, ..., g W_n\}.$$ Let $\{W_1, ..., W_n\}, \{V_1, ..., V_n\}\in F_n$ and choose basis elements of $w_i$ and $v_i$ for each $W_i$ and $V_i$ respectively so that $\{w_i\}_{i=1}^n$ and $\{v_i\}_{i=1}^n$ are orthonormal basis of $\C^n$. Recall from elementary algebra that the transition matrix mapping $\{w_i\}$ onto $\{v_i\}$ is unitary. Therefore this (smooth) action of $U(n)$ on $F_n$ is transitive. Moreover, the isotropy group of $e$ is the torus $T$. So by Theorem \ref{theorem} $$U(n)/T \cong F_n.$$
	Any element $\{W_i\}_{i=1}^n \in F_n$ can be identified with a set of orthogonal projections $\{P_i\}_{i=1}^n$ for $P_i:\C^n\to W_i$.  By orthogonality, $P_iP_j = 0$ if $i\neq j$ and $\sum_{i=1}^n P_i = 1$. Therefore elements of $U(n)/T \times T$ can be identified with pairs $(P, t)$ where $P = (P_1, ..., P_n)$ are orthogonal projections and $t = \text{diag}(p_1(t), ..., p_n(t))$. The $p_i(t)$ can be thought of as the eigenvalues of a unitary matrix $g$, with $P_i$ being the orthogonal projections onto the $p_i(t)$-eigenspace. By requiring $p_1(t)\cdots p_n(t) = 1$, pairs $(P, t)$ can be identified with $\su\times T$.  With this description in mind, the Weyl map $p: SU(n)/T\times T\to SU(n)$ becomes \begin{align} \label{weylmapdescription} (P, t)\mapsto \sum_{i}p_i(t)P_i \end{align} To see this, consider the identification \begin{gather*}
	T\times \su \to T\times F_n\\
	(t, gT) \mapsto (t, gE_1g^{-1}, ..., gE_ng^{-1}).
	\end{gather*} Then $$p(t, gT) = gtg^{-1} = g\left(\textstyle \sum_{i=1}^n p_i(t)E_i\right)g^{-1} =  \textstyle \sum_{i=1}^n p_i(t) \left(gE_ig^{-1}\right)$$ so $p(t, gE_1g^{-1},..., gE_ng^{-1}) =   \textstyle \sum_{i=1}^n t_i \left(gE_ig^{-1}\right)$, giving us the description of the Weyl map on $T\times F_n$ above. 
	\subsection{Connective structure on the cup product bundle gerbe} 
	In this section we aim to compute blah blah blah  in three steps. Herein we shall refer to a bundle gerbes $ \left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i\in \{1, ..., n\}$ as the \textit{$i$-th cup product bundle gerbe}.
	% Recall the line bundle $\widetilde{J}_i\to \su$ with $\widetilde{J}_i := SU(n)\times \C /\sim_{\widetilde{p}_i}$ defined in Example \ref{ex 1}. 
	\begin{proposition}\label{curvaturetwoform}
		For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla^{{J}_i}$ on ${J}_i\to \su$ with curvature $F_{\nabla_{{J}_i}} = \textup{tr}(P_idP_idP_i)$ for $P_i:\su\times \C^n\to J_i $ orthogonal projection which is point-wise a map $P_i(gT): \{gT\} \times \C^n\to (J_i)_{gT} \subset \{gT\}\times \C^n$. 
	\end{proposition}
	
	%\begin{proposition}
	%	For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla_i$ on $J_i\to T\times \su$ with curvature $$F_{\nabla_i} = \text{tr}(P_idP_idP_i)$$ for $P_i:\su\times \C\to J_i$ orthogonal projection. 
	%\end{proposition}
	\begin{proof} To show this, we will utilise Example \ref{linebundleconnection}. To do so, let us first understand ${J}_i$ as a subbundle of a trivial bundle of rank $n$. Now, ${J}_i$ is a subbundle of the $SU(n)$-homogeneous line bundle $\frac{SU(n)\times \C^n}{T}\to \su$. The latter is isomorphic to the trivial bundle $\su \times \C^n \to \su$ by Theorem \ref{thrmbundles}. Therefore by Example \ref{linebundlecurvature} projection of the trivial connection gives us a connection $\nabla_{{J}_i}:= P_i(d)$ on ${J}_i\to \su$ with curvature two form $F_{\nabla_{{J}_i}} = \text{tr}(P_idP_idP_i)$. \end{proof}
	
	\begin{remark}\label{remark curvatureofJ} 
		Recall that (abusing notation) we have the line bundle $J_i \to T\times \su$ defined by pulling back $J_i\to \su$ along $T\times \su\to \su$. Using that there is an induced pullback connection on $J_i\to T\times \su$, it is not difficult to show by the previous proposition that the pullback connection on $J_i\to T\times \su$ has curvature $\text{tr}(P_idP_idP_i)$ for $P_i: \su \times T\times \C^n \to J_i$ orthogonal projection. Just as we abuse notation with the line bundles $J_i$, we abuse notation and write the curvatures of the connections on these respective line bundles as $\text{tr}(P_idP_idP_i)$ despite the projections being defined on different spaces. 
	\end{remark}
	
	%
	%\begin{corollary}\label{curvatureofJ} 
	%	For each $i=1, ..., n$ there is a canonical line bundle connection $\nabla^{J_i}$ on $J_i\to T\times \su$ with curvature $$F_{\nabla^{J_i}} = \textup{tr}(P_idP_idP_i) $$ for $P_i:T\times \su \times \C \to J_i$ orthogonal projection.
	%\end{corollary}
	%\begin{proof}
	%Recall that $J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1} \widetilde{J}_i$ for $\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su \to \su$ projection. So we can pullback the connection $\nabla^{\widetilde{J}_i}$ on $\widetilde{J}_i\to \su$ defined above to obtain the connection $$\nabla^{J_i}:= \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}\nabla^{\widetilde{J}_i}$$ on $J_i\to T\times \su$. This connection has curvature two form $F_{\nabla^{J_i}} = \pi_{\smath{ \dfrac{SU(n)}{T} } }^{*} F_{\nabla^{\widetilde{J}_i}}$. Pulling back the curvature two form $F_{\nabla^{\widetilde{J}_i}}$ from Proposition \ref{curvaturetwoform} is equivalent to pulling back the orthogonal projections $\su \times \C\to \widetilde{J}_i$ in its definition along $\su\times T \times \C\to \su\times \C$, giving us the result. {\textcolor{red}{is this right?}} 
	%\end{proof}
	
	
	\begin{proposition}\label{existsconnectiononcup} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Let $f:M\to S^1$ be a smooth map. For each $k\in \Z$ define the projection $$\pi_k: \{k\}\times f^{-1}(\R)\to M.$$Then on the cup product bundle gerbe $\left(P\cup f, f^{-1}(\R), M\right)$ there is a bundle gerbe connection $\nabla_{P\cup f}$ with curvature two-form $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ on connected components of $\Z\times f^{-1}(\R) \cong f^{-1}(\R)^{[2]}$.  
	\end{proposition}
	\begin{proof}
		Over $\{k\}\times f^{-1}(\R)$, $P\cup f = \pi_k^{-1}(P)^k$, so $\pi_k^{-1}(\nabla)^k$ defines a connection on connected components $\{k\}\times f^{-1}(\R)$ of $\Z\times f^{-1}(\R)$, hence defines a global connection $\nabla_{P\cup f}$ on $P\cup f \to \Z\times f^{-1}(\R)$. This is a bundle gerbe connection since, for $(n, t_1, t_2, t_3)\in f^{-1}(\R)^{[2]}$ and $m$ the bundle gerbe multiplication on $P\cup f$, $$m\left((P_n)^{t_1-t_3}\otimes (P_n)^{t_1-t_2}\right) = (P_n)^{t_1-t_3}$$ implies $$m(\nabla^{t_1-t_2}\otimes 1 + 1\otimes \nabla^{t_1-t_2}) = \nabla^{t_1-t_3}, $$ which is precisely what it means for $\nabla_{P\cup f}$ to be a bundle gerbe connection in this instance. It then follows immediately by Proposition \ref{constructingconnections} that $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ for all $k\in \Z$.
	\end{proof}
	\begin{example}\label{connectiononJ}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i= 1, ..., n$. For each $k\in \Z$ let $$\pi_{k,i}: \{k\}\times p_i^{-1}(\R)\to T\times \su $$ be projection and $\nabla_{J_i}$ a connection on $J_i\to T\times \su$. Then by the previous proposition, there is a bundle gerbe connection $\nabla_{J_i\cup p_i}$ on the $i$-th cup product bundle gerbe with two-curvature $$ F_{\nabla_{J_i\cup p_i}}\big |_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_{k,i}^{*}F_{\nabla_{J_i}}.$$
	\end{example}
	
	
	%\begin{proposition}\label{connectiononJ}
	%Consider the $i$-th cup product bundle gerbe for $i\in \{1, ..., n\}$.  Let $k\in \Z$, and define the projection $$\pi_{k}: \{k\}\times p_i^{-1}(\R) \to \su $$ onto the $\su$ element of $p_i^{-1}(\R)$. There is a bundle gerbe connection $\nabla^{\cup_i}$ on the $i$-th cup product bundle gerbe with curvature two-form $$F_{\nabla^{\cup_i}} \big\rvert_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_k^{-1}\left(F_{\nabla^{\widetilde{J}_i}}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)\cong p_i^{-1}(\R)^{[2]}$.
	%\end{proposition}
	%
	%\begin{proof} Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ as in Remark \ref{isocup}. To define a line bundle connection on $J_i\cup p_i\to \Z\times \left(\widetilde{p}_i\right)^{-1}(\R) \times \su$ it suffices to define a connection on connected components $U_k:= \{k\}\times p_i^{-1}(\R)$ for $k\in \Z$. Recall $\widetilde{J}_i\to \su$ has line bundle connection $\nabla^{\widetilde{J}_i}$. Hence $\nabla^{\widetilde{J}_i^k}$ is a connection on $\widetilde{J_i}^k \to \su$. So $\pi_k^{-1}\nabla^{\widetilde{J}_i}$ defines a connection on $\pi_k^{-1}\widetilde{J}_i^k \cong J_i\cup p_i \big\rvert_{\{k\}\times p_i^{-1}(\R)}$ This is a bundle gerbe connection because $\nabla^{\widetilde{J}_i}$ is. It follows immediately that the two curvature of the connection $\pi_k^{-1}\left(\nabla^{\widetilde{J}_i^k}\right)$ is $k\cdot \pi_k^{-1}(F_{\nabla^{\widetilde{J}_i}})$ by Proposition \ref{constructingconnections}. \end{proof}
	\begin{remark}
		By Proposition \ref{tensorproductconnection} and Proposition \ref{constructingconnections}, there is a bundle gerbe connection $\nabla^{\otimes \cup}$ on  $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ with curvature two form $$F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{*}\left(F_{\nabla^{{J}_i}}\right)  $$ over connected sets $\{(k_1, ..., k_{n-1})\}\times \R^{n-1}\times \su \subset \Z^{n-1}\times \R^{n-1}\times \su \cong \left(\R^{n-1}\times \su\right)^{[2]}$ with $k_n := -k_1 - \cdots - k_{n-1}$. By Remark \ref{remark curvatureofJ} this can be written as $$ F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{-1}\left(\text{tr}(P_idP_idP_i)\right)$$ for $P_i: T\times \su \times \C^n \to {J}_i$ orthogonal projection. 
	\end{remark}
	%\text{}\\ 
	%of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$
	
	
	
	
	
	\begin{proposition} \label{curvaturetheorem1} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Consider the cup product bundle gerbe $(P\cup f, f^{-1}(\R), M)$ defined for $f:M\to S^1$ a smooth map. Let $\pi:f^{-1}(\R)\to M$ be the surjective submersion in this bundle gerbe and $\nabla_{P\cup f}$ the bundle gerbe connection from Proposition \ref{existsconnectiononcup}. Define a two-form $h$ on $f^{-1}(\R)$ by $$h(m, x) = x \cdot \pi^*F_\nabla. $$ Then 
		\begin{enumerate}[(1),font=\upshape]
			\item the two form $h$ satisfies $\delta(h) = F_{\nabla_{P\cup f}}$, so $h$ is a curving for the bundle gerbe connection $\nabla_{P\cup f}$;
			\item the three-curvature $\mu \in \Omega^3(M)$ of the bundle gerbe connection $\nabla_{P\cup f}$ is given by $$\mu =  \frac{1}{2\pi}\, f^{*}(d\theta) \wedge F_{\nabla} $$ for $\theta \in (0,2\pi)$ the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class of $(P\cup f, f^{-1}(\R), M)$ is 
			$$\frac{-i}{4\pi^2}\, f^{*}(d\theta) \wedge F_{\nabla}.$$ 
		\end{enumerate}
	\end{proposition}
	
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	
	\begin{proof} Let us first compute $\delta(h)$. Now, for $(m, x, x') \in f^{-1}(\R)^{[2]}$
		
		\begin{align*}
		\delta(h)\big\rvert_{(m, x, x')} &= \pi_1^{-1} h \big \rvert_{(m, x, x')}   - \pi_2^{-1}h\big\rvert_{(m, x, x')} \\ 
		&=  h\big\rvert_{(m, x')}\circ d\pi_1-  h\big\rvert_{(m, x)}\circ d\pi_2
		\end{align*}
		By noting that $T\Z = 0$ and $f^{-1}(\R)^{[2]} \cong \Z \times f^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla}\big\rvert_{(m, x')} = \pi^{-1}F_{\nabla}\big\rvert_{(m, x)}$. Therefore at a point $(m, x, x')\in f^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
		\delta(h) &= k \cdot \pi^{-1}F_{\nabla}\circ d\pi_1 \big |_{\{k\}\times f^{-1}(\R)}\\ 
		&= k\cdot (\pi\circ\pi_1 |_{\{k\}\times f^{-1}(\R)})^{-1}F_{\nabla}\\
		&= k\cdot \pi_k^* F_{\nabla}\\
		&= F_{\nabla_{P\cup f}}\big |_{\{k\}\times f^{-1}(\R)}.
		\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu\in \Omega^3\left(M\right)$ is defined implicitly by $$dh = \pi^{*}\mu.$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (f\circ \pi)^{*}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
		dh&= d\left(x \cdot \pi^{*}F_\nabla\right)\\
		&= dx \wedge \pi^{*}F_{\nabla}\\
		&= \frac{1}{2\pi} \, \pi^{*}\left(f^{*}(d\theta)\wedge F_{\nabla}\right). 
		\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	
	\begin{example}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ with surjective submersion $\pi_i: p_i^{-1}(\R)\to T\times \su$  and connection and curvature $\nabla^{\cup_i}$, $F_{\nabla^{\cup_i}}$. By the previous proposition, this bundle gerbe has curving $h_i \in \Omega^2(p_i^{-1}(\R))$ given by $$h_i(t, gT, x) = x\cdot \pi_i^* F_{\nabla^{J_i}}$$ and three-curvature $\mu_i\in \Omega^3(T\times \su)$ given by $$\mu_i = \frac{1}{2\pi}\, p_i^*(d\theta) \wedge F_{\nabla^{J_i}}.$$ Moreover, the Dixmier-Douady class of the $i$-th cup product bundle gerbe is $$-\frac{i}{2\pi^2}\, p_i^*(d\theta)\wedge F_{\nabla^{J_i}}. $$
	\end{example}
	
	
	%
	%
	%\begin{proposition}
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	%	\end{proposition}
	%\begin{proof} Let us first compute $\delta(h_i)$. Now, for $(t, gT, x, x') \in p_i^{-1}(\R)^{[2]}$ \begin{align*}
	%\delta(h_i)\big\rvert_{(t, gT, x, x')} &= \pi_1^{-1} h_i \big \rvert_{(t, gT, x, x')}   - \pi_2^{-1}h_i \big\rvert_{(t, gT, x, x')} \\ 
	%&=  h_i\big\rvert_{(t, gT, x')}\circ d\pi_1-  h_i\big\rvert_{(t, gT, x)}\circ d\pi_2
	%\end{align*}
	%By noting that $T\Z = 0$ and $p_i^{-1}(\R)^{[2]} \cong \Z \times p_i^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x')} = \pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x)}$. Therefore at a point $(t, gT, x, x')\in p_i^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
	%\delta(h_i) &= k \cdot \pi^{-1}F_{\nabla^{J_i}}\circ d\pi_1\\ 
	%&= k\cdot (\pi\circ\pi_1)^{-1}F_{\nabla^{J_i}}\\
	%&= k\cdot \left(\pi_{\smath{ \dfrac{SU(n)}{T} } }\circ \pi \circ \pi_1\right)^{-1} F_{\nabla^{\widetilde{J}_i}}\\
	%&= k \cdot \pi_k^{-1}F_{\nabla^{\widetilde{J}_i}}\\
	%&= F_{\nabla^{\cup_i}}.
	%\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu_i \in \Omega^3\left(T\times \su\right)$ is defined implicitly by $$dh_i = \pi^{-1}(\mu_i).$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (p_i\circ \pi)^{-1}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
	%dh_i &= d\left(x \cdot \pi^{-1}\left(F_{\nabla^{J_i}}\right)\right)\\
	%&= dx \wedge \pi^{-1}\left(F_{\nabla^{J_i}}\right)\\
	%&= \pi^{-1}\left(\textstyle \frac{1}{2\pi} p_i^{-1}(d\theta)\wedge F_{\nabla^{J_i}}\right). 
	%\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	% Let us first construct the connection on the cup product bundle gerbe. Consider a connected open subset $U\subseteq f^{-1}(\R)^{[2]}$. Recall that $f^{-1}(\R)^{[2]}$ consists of triples $(m, t_1, t_2) \in M\times \R^2$ satisfying $f(m) = [t_1] = [t_2]$. The difference map $d:\R^{[2]}\to \Z$ is continuous and therefore constant on connected components. Therefore for all $(m, t_1, t_2) \in U$, $t_1-t_2 = k$ for some fixed integer $k$. {\textcolor{red}{need to think about connectedness of product I'm getting confused}} Therefore $$(P\cup f)|_U = P^k|_U.$$ Let $\nabla$ be a connection on $P\to M$. Then $\nabla^k$ is a connection on $(P\cup f)|_{U_k}$. Since we can do this for all connected subsetes $U_k$ of $f^{-1}(\R)^{[2]}$, we have a connection $\nabla^{P\cup f}$ on all of $P\cup f$. To see that this is a bundle gerbe connection, recall that bundle gerbe multiplication on $P\cup f$ is given by $$(P_m)^{t_2-t_3} \otimes (P_m)^{t_1-t_2} = (P_m)^{t_1-t_3}.$$ Certainly $$\nabla^{t_1-t_2}\otimes \nabla^{t_1-t_2} = \nabla^{t_1-t_3}$$ so this connection respects the bundle gerbe multiplication.\text{}\\ \text{}\\ 
	%\indent Let $\{U_\alpha\}_{\alpha \in I}$ be an open cover of $M$ such that for each $U_\alpha$ there exists a non-vanishing section $s_\alpha: U_\alpha\to P$. Then there exists connection one forms $A_\alpha \in \Omega^1(U_\alpha)$ for which the connection $\nabla$ on $P\to M$ satisfies $$\nabla s_\alpha = A_\alpha s_\alpha.$$ Let us now find an expression for the connection one forms on $P\cup f\to f^{-1}(\R)^{[2]}$. It suffices to find the connection one forms corresponding to the connection $\nabla^k$ on $P^k|_{U_k}\to {U_k}$ by the above discussion. It is easy to verify that on $P^k|_{U_k}\to {U_k}$ the connection one forms are $$kA_\alpha \in \Omega^1(U_k\cap U_\alpha).$$ Therefore locally $F_{\nabla^k} = kdA_\alpha$, and since $F_{\nabla^{P\cup f}|_{U_k}} = F_{\nabla^k}$, this gives us a local expression for $F_{\nabla^{P\cup f}}$. Next, define $f\in \Omega^2(f^{-1}(\R))$ by $f(m, x) = x\cdot \pi^* F_\nabla$ where $\pi:f^{-1}(\R) \to M$ is the projection map. It can be verified that $f$ is a curving for $kA_\alpha$, that is, (locally) $\delta(f) = kdA_\alpha$ (where we are really pulling the latter two form back by the projection $f^{-1}(\R)^{[2]}\to M$). We can now compute the three-curvature. Now,  \begin{align*}
	%df = d(x\pi^*F_\nabla) = dx\wedge \pi^*F_\nabla = \pi^*(f^* d\theta \wedge F_\nabla)
	%\end{align*} 
	%{\textcolor{red}{really confused with this entire thing. struggling to write this concisely without using all of the pullbacks hidden in here. Also don't understand why we have $d\theta$ here when we actually want it to be $\lambda_k^*d\theta$. }}
	\begin{corollary}\label{corollary data on cup prod} 
		Consider the tensor product of the cup product bundle gerbes$$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$$ with connection $\nabla^{\otimes \cup}$ and curvature $F_{\nabla^{\otimes \cup}}$. Let $h_i$ and $\mu_i$ be the curving and three curvature respectively of the $i$-th cup product bundle gerbe with connection $\nabla^{\cup_i}$. Let $P_i$ be orthogonal projection $T\times \su\times \C^n\to J_i$. Then \begin{enumerate}[(1),font=\upshape]
			\item the two form $$h := \sum_{i=1}^n h_i$$ on $\R^{n-1}\times \su$ satisfies $\delta(h) = F_{\nabla^{\otimes \cup}}$, ie. $h$ is a curving for the connection $\nabla^{\otimes \cup}$;
			\item the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1} dp_i\wedge \textup{tr}(P_idP_idP_i)$$for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class is $$\frac{-i}{4\pi^2}\sum_{i=1}^n p_i^{-1} d p_i\wedge \textup{tr}(P_idP_idP_i).$$ 
		\end{enumerate}
	\end{corollary}
	\begin{proof}  By Theorem \ref{curvaturetheorem1}, the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi}\sum_{i=1}^n p_i^{-1}(d\theta)\wedge \text{tr}(P_idP_idP_i)$$ and the Dixmier-Douady class is $\frac{1}{2\pi i } \mu$. Using the coordinates $\theta = -i\log$ on $S^1$, we find that the pullback of $d\theta$ by $p_i: T\times \su \to S^1$ is $$p_i^{-1}(d\theta) = -i\frac{dp_i}{p_i}.$$ Therefore the three curvature of $\nabla^{\otimes \cup}$ can be rewritten as $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1}dp_i \text{tr}(P_idP_idP_i),$$ and similarly for the Dixmier-Douady class.\end{proof}
	
	%I am proving the following proposition. 
	%\begin{proposition}\label{connectiononJ}
	%	Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ for each $i=1, ..., n$. Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ and denote the surjective submersion $\Z\times p_i^{-1}(\R)\to T\times \su$ by $\pi$. Then for each $i=1, ..., n$, there is a bundle gerbe connection $\nabla^{J_i\cup p_i}$ on $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ with curvature two-form given by $$F_{\nabla^{J^i\cup p_i}} \big\rvert_{\{n\}\times p_i^{-1}(\R)} = n \cdot \pi^{-1}\left(F_{\nabla_i}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)$.
	%\end{proposition}
	
%	\textit{Proof}. Consider a connected component $U_n:= \{n\}\times p_i^{-1}(\R)$ of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$


==> chapter3-5/CHP5.tex <==
%!TEX root = ../thesis.tex

	
	\chapter{Cup product bundle gerbe}
	In the proceeding example we construct the \textit{cup product} bundle gerbe, which will be central to our research. The definition of the cup product bundle gerbe is motivated by the cup product map of \v{C}ech cocycles. Given sheaves of abelian groups $F$ and $G$, the cup product
	$$\cup: C^p(\mathcal{U}, F)\otimes C^{q}(\mathcal{U}, G) \to C^{p+q}(\mathcal{U}, F\otimes G)$$ is defined by mapping  $(\underline{\alpha}, \underline{\beta})\mapsto \underline{\alpha}\cup \underline{\beta}$ where $$(\underline{\alpha}\cup \underline{\beta})_{i_0, ..., i_{p+q}} := \alpha_{i_0, ..., i_p}\otimes \beta_{i_q, ..., i_{p+q}}. $$ In particular, taking $F = \Z(1)_D$, $Q = \Z(2)_D$, $p=1$ and $q=2$, the cup product induces a map of \v{C}ech hypercohomology groups, and hence of sheaf hypercohomology groups, \begin{align}\label{eqn cup product} \cup: H^1(M, \Z(1)_D)\otimes H^{2}(M, \Z(2)_D) \to H^{3}(M, \Z(3)_D).\end{align} 
	Recall that smooth maps $f:M\to U(1)$, line bundles with connection, and bundle gerbes with connective structure are classified by $H^1(M, \Z(1)_D)$, $H^{2}(M, \Z(2)_D)$, and $H^3(M, \Z(3)_D)$ respectively (Remark \ref{remark deligne cohomology of line bundles and functions}). Therefore by Equation \ref{eqn cup product} we expect the cup product to define a bundle gerbe $(f\cup L, Y, M)$ given a map $f: M\to U(1)$ and a line bundle $L\to M$ with connection. Of course, the Deligne class of $(f\cup L, Y, M)$ will then equal the cup product of Deligne classes of $f$ and $L\to Y$.
	
	
	This construction describes how a bundle gerbe can be formed given a smooth map $M\to S^1$ and a line bundle over $M$. The set up is as follows. Let $M$ be a smooth manifold, $\pi: P\to M$ be a line bundle, and $f:M\to S^1$ be a smooth map. Let $\R\to S^1$ be the principal $\Z$-bundle with projection $x\mapsto [x]$ the quotient map by $\Z$. The given information is depicted below.% As we shall see, the map $f:M\to S^1$ allows us to construct a bundle gerbe over $M$ from a line bundle over $M$. 
	
	\begin{center} 
		\begin{tikzcd}
			P  \arrow[swap]{d}{\pi}       
			&\R \arrow{d}{[\cdot]} \\
			M  \arrow[swap]{r}{f}
			&S^1
		\end{tikzcd} 
		\text{}\\ \text{}\\ { \color{red}{Label this diagram }} 
	\end{center}
	By pulling back $\R \to S^1$ along $f$, we obtain a $\Z$-bundle $f^{-1}(\R)$ over $M$. The space $f^{-1}(\R)$ consists of pairs $(m, t) \in M\times \R$ with $f(m) = [t]$. By Example \ref{fibreproductexample} the second fibre product of $f^{-1}(\R)$ consists of triples $(m, t_1, t_2)\in M\times \R\times \R$ with $f(m) = [t_1]=[t_2]$. Let $d: f^{-1}(\R)^{[2]}\to \Z$ be the difference map $d(m, t_1, t_2) = t_1-t_2$. Let $\pi_M: f^{-1}(\R)^{[2]} \to M$ be projection. Define a line bundle $P\cup f\to f^{-1}(\R)^{[2]}$ by $$P\cup f := \pi_M^{-1}\left(P\right)^d$$ using the notation from Example \ref{powerlinebundles}. To be completely explicit, for $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$, $$(P\cup f)_{(m, t_1, t_2)} = (P_m)^{d(m,t_1, t_2)}.$$ We claim the triple $(P\cup f, f^{-1}(\R), M)$ is a bundle gerbe. The space $P\cup f$ is indeed equipped with a natural bundle gerbe multiplication. Let $(m, t_1, t_2, t_3) \in Y^{[3]}$.  Then \begin{align*}
	\pi_1^{-1}(P\cup f)\otimes \pi_3^{-1}(P\cup f)_{(m, t_1, t_2, t_3)} 
	&= (P_m)^{t_2-t_3}\otimes (P_m)^{t_1-t_2}\\
	&= (P_m)^{t_1-t_3}\\
	&= \pi_2^{-1}(P\cup f)_{(m, t_1, t_2, t_3)}. 
	\end{align*} This map is certainly a smooth isomorphism of line bundles. Associativity of the bundle gerbe multiplication  follows from associativity of the tensor product of line bundles. 
	\begin{definition}  Given a smooth manifold $M$, a smooth map $f: M\to S^1$, and a line bundle $P\to M$, the triple $(P \cup f, f^{-1}(\R), M)$ constructed above is a bundle gerbe, called the \textit{cup product bundle gerbe}. \end{definition} {\color{red}{give motivation for name by talking about DD class}} 
	\begin{center} 
		\begin{align*}
		\begin{array}{ccc}
		P \cup f      &              \\
		\downarrow &               \\
		f^{-1}(\R)^{[2]}   & \stackrel{}{\dra} f^{-1}(\R) \\
		&                   \downarrow  \\
		&                    M      \\
		\end{array}
		\end{align*}
		{\color{red}{label diagram}} 
	\end{center}
	\begin{remark}\label{isoZ}
		Note that $f^{-1}(\R)^{[2]} \cong f^{-1}(\R)\times \Z$. This follows since $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$ if $f(m) = [t_1] =[t_2]\in S^1$. The latter equality holds if and only if $t_1-t_2\in \Z$. So by identifying an element $(m, t_1, t_2)\in f^{-1}(\R)^{[2]}$ with $(m, t_1, t_1-t_2) \in  f^{-1}(\R)\times \Z$ we obtain the desired diffeomorphism. 
	\end{remark}
	\begin{example}\label{ex 1}
		In this example we look at a specific instance of the cup product bundle gerbe. We shall first define a line bundle over $T\times \su$, and will obtain from this a bundle gerbe over $T\times \su$ using the cup product construction. Let $T$ be the maximal torus of $SU(n)$ defined by $$T := \{\text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}) : \ x_1 + \cdots + x_n = 0\}\cong \left(S^1\right)^{n-1}. $$ For $i = 1, ..., n$, define the group homomorphism $$ {p}_i: T\to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n})  \mapsto e^{2\pi i x_i}.$$ For each $i=1, ..., n$, define a line bundle $\pi: {J}_i \to \frac{SU(n)}{T}$ by $${J}_i = SU(n)\times \C/\sim_{{p}_i}, $$ where $(s, z)\sim_{{p}_i} (st, {p}_i(t^{-1})z)$ for all 
		$(s, z) \in SU(n)\times U(1)$ and $t\in T$.  Denote equivalence classes in $J_i$ by $[\cdot, \cdot]_{p_i}$. It follows  that the projection $\pi: [(s, z)] \mapsto sT$ is a well-defined surjective submersion. We abuse notation and denote the pullback of $J_i$ along the projection $T\times \su \to \su$ by $J_i\to T\times \su$ throughout this work. Consider the map $$p_i: T\times\su \to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}, gT)\mapsto e^{2\pi i x_i}$$ defined for $i=1, ..., n$. 
		
		
		%	Consider the projection $$\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su\to \su$$ and define a line bundle ${J}_i \to T\times \su$ by $$J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}{J}_i'.$$
		%	%Using the constant identity-valued map $\textbf{1}_n: J_i\to T$, we can consider $J_i$ as a line bundle over $T\times \su$ with projection $1\times \pi$. 
		The elements that will be used to construct the cup product bundle gerbe are depicted below. 
		
		\begin{figure}[h!] 
			\begin{center} 
				\begin{tikzcd}
					J_i  \arrow[swap]{d}{}      
					&\R   \arrow{d}{[\cdot]}  \\
					T\times \frac{SU(n)}{T}\arrow[swap]{r}{p_i}
					&S^1
				\end{tikzcd}  \caption{Cup product bundle gerbe set up}
				\label{fig:pb1} \end{center}\end{figure} 
		%$J_{i,  {\smath{ \dfrac{SU(n)}{T} } }}, J_{i, T\times {\smath{ \dfrac{SU(n)}{T} } }}$ {\textcolor{red}{FINISH NEATENING UP NOTATION}}	Lastly, by pulling back $\R\to S^1$ by $p_i$ as before 
		Using the construction defined about, for each $i=1, ..., n$, we obtain a cup product bundle gerbe $$\left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$$ 
		%Consider the projection $$\pi_{T\times {\smath{ \dfrac{SU(n)}{T} } }}: p_i^{-1}(\R)^{[2]}\to T\times \su$$, 
		where, for any $(x_1, x_2,t,sT) \in p_i^{-1}(\R)^{[2]}$, we have $$(J_i \cup p_i)_{(x_1, x_2, t, sT)} = \left({J}_i \right)_{sT}^{x_1-x_2}.$$ %Since this fibre is independent of $t \in T$, we may sometimes abuse notation and write this fibre as $(J_i  \cup p_i)_{
		%	(x_1, x_2,sT)}$. 
		%$$(L_i\cup \varphi_i, \R^{n-1}\times  \tfrac{SU(n)}{T}, T\times  \tfrac{SU(n)}{T}). $$ {\color{red}{refer to figure}}   $$ \begin{array}{ccc}
		%L_i\cup \lambda_i         &          &        \\
		%\downarrow &         &         \\
		%\R^{n-1}\times \tfrac{SU(n)}{T}\times \Z  & \stackrel{}{\dra} &  \R^{n-1}\times \tfrac{SU(n)}{T} \\
		%&               &      \downarrow \\
		%&               &       T\times  \frac{SU(n)}{T}        \\
		%\end{array} $$
	\end{example} 
	In the following example, the product of these $n$ bundle gerbes is formed to construct a single bundle gerbe over $T\times \su$. The resulting bundle gerbe will be central to our research question. 
	\begin{remark}\label{isocup}
		%By remark \ref{isoZ}, we see that $p_i^{-1}(\R)^{[2]}\cong p_i^{-1}(\R)\times \Z$. We can also understand these spaces in terms of the original projection map $\widetilde{p}_i: T\to S^1$ as $$p_i^{-1}(\R)\cong \left(\widetilde{p}_i\right)^{-1}(\R)\times \su$$ and $$p_i^{-1}(\R)^{[2]} \cong \Z\times \left(\widetilde{p}_i\right)^{-1}(\R)\times \su.$$ 
		We can write the space $p_i^{-1}(\R)$ explicitly as $$p_i^{-1}(\R) = \left \{(t, gT, x)\in T\times \su \times \R \ \big \rvert \ t_i = [x]\right\}.$$ 
	\end{remark}
	\begin{proposition}\label{cupprodisequivariant} 
		The cup product bundle gerbes $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ defined above are $SU(n)$-equivariant for each $i=1, ..., n$. 
	\end{proposition}
	\textit{Proof}. Let us define the $SU(n)$ action on each of the spaces present in our bundle gerbe. On $T\times \su$, $SU(n)$ acts by $$g\cdot (t, hT) := (t, ghT). $$ On $p_i^{-1}(\R) = \left \{(x, t, hT) \in \R\times T\times \su \ | \ p_i(t) = [x]\right\}$, $SU(n)$ acts by $$g\cdot (x, t, hT) := (x, t, ghT), $$ and similarly for $p_i^{-1}(\R)^{[2]}$. Finally, for a standard element $\otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} \in (J_i\cup p_i)_{(x_1, x_2, hT)}$ the $SU(n)$-action is defined by $$g\cdot \otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} := \otimes_{j=1}^{x_1-x_2} [gh, v_j]_{p_i}. $$ This can be extended by linearity to define an action on any element in $J_i\cup p_i$. With these actions, $SU(n)$-equivariance of the bundle gerbe follows easily. 
	
	\begin{example}\label{exxx}
		Consider the bundle gerbes $\left(J_i \cup p_i, p_i^{-1}(\R), T\times \frac{SU(n)}{T}\right)$ for $i= 1, ..., n$ as in Example \ref{ex 1}. To describe the product of these $n$ bundle gerbes, we must first understand the fibre product $$H = p_1^{-1}(\R) \times_{T\times \frac{SU(n)}{T} }\times \cdots \times_{T\times \frac{SU(n)}{T}} p_n^{-1}(\R).$$ Since the projection from $p_i^{-1}(\R) \subseteq \R\times \left(T\times \su\right)$ to $  T\times \su$ is simply projection onto the second factor, it is clear that $$H \cong \left\{(x_1, ..., x_n, t, gT)\in \R^n \times T\times \tfrac{SU(n)}{T} \ \big\rvert\ [x_i] = p_i(t)\ \forall \  i = 1, ..., n \right\}.$$ Since the product of the diagonal entries of $t$ equals one, the condition that $[x_i] = p_i(t)$ for each $i = 1, ..., n$ can equivalently be stated as $x_1 + \cdots + x_n \in \Z$. Using this condition, and noting that $t = \text{diag}([x_1], ..., [x_n])$,  we find $$H \cong \left\{(x_1, ..., x_n, gT) \in \R^n \times \tfrac{SU(n)}{T} \ \big\rvert \ \textstyle \sum_{i=1}^n x_i \in \Z\right\}.$$ Let $W := \{(x_1, ..., x_n) \in \R^n :  \textstyle \sum_{i=1}^n x_i \in \Z\}.$ Then $H \cong W
		\times \tfrac{SU(n)}{T}.$ We remark that under this identification, the surjective submersion $H\to T\times \su$ becomes $$(x_1, ..., x_n, gT) \mapsto (\text{diag}([x_1], ..., [x_n]), gT)$$ when written as a map $W\times \su \to T\times \su$.  Therefore the tensor product from $i=1, ..., n$ of the bundle gerbes from Example \ref{ex 1} can be written as \begin{align} \label{eqn} \left(\Motimes_{i=1}^n J_i \cup p_i, W\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right). \end{align} 
	\end{example} 
	In some instances, a bundle gerbe $(P, Y, M)$ can equivalently be viewed as a bundle gerbe $(P|_{X^{[2]}}, X, M)$ for some submanifold $X\subseteq Y$. This is in fact a result of the following theorem.
	
	\begin{theorem}[\cite{stableiso}] \label{stable iso} 
		Let $\pi_1: Y\to M$, $\pi_2: X\to M$ be surjective submersions, and $f: X\to Y$ a morphism of surjective submersions, ie. $\pi_1\circ f = \pi_2$. Then a bundle gerbe $(P, Y, M)$ is stably isomorphic to $(f^{-1}(P), X, M)$. 
	\end{theorem} 
	An important consequence of this theorem occurs when $f$ is the inclusion of a submanifold into a manifold. The resulting corollary makes precise when a bundle gerbe $(P, Y, M)$ can equivalently be viewed as the bundle gerbe $(P|_{X^{[2]}}, X, M)$ for a submanifold $X\subset Y$. 
	
	
	\begin{corollary}\label{ex 2} 
		Consider a bundle gerbe $(P, Y, M)$ and a submanifold $X\subset Y$ such that $\pi|_X:X\to M$ is a surjective submersion. Let $\iota: X\to Y$ be inclusion. Then $\pi\circ \iota = \pi|_X$, therefore by Theorem \ref{stable iso} $(P, Y, M)$ is stably isomorphic to $(P|_{X^{[2]}}, X, M)$. 
	\end{corollary}
	This Corollary is most useful when the submanifold $X$ of $Y$ simplifies calculations on the bundle gerbe.  This is in fact the case for the bundle gerbe (\ref{eqn}), where the space $W \times \su$ can be replaced by the (simpler) space $\R^{n-1}\times \su$. We return to Example \ref{exxx} to make this precise. \\
	
	\noindent\textbf{Example 1.32. (Continued)} Let us justify why the space $W\times \su$ present in the bundle gerbe (\ref{eqn}) can be replaced with the space $\R^{n-1}\times \su$. First, note that $\R^{n-1}$ can be viewed as a submanifold of $W$ under the identification $$\R^{n-1} \cong \left\{(x_1, ..., x_n) \in \R^n \ \big\rvert \  \textstyle\sum_{i=1}^n x_i = 0\right\} \subseteq W.$$ Recall that the projection $W\times \su \to T\times \su$ is defined by $$ (x_1, ..., x_{n}, gT) \mapsto \left(\text{diag}\left([x_1], ...,  [x_n]\right), gT\right).$$ This map remains a surjective submersion when restricted to $\R^{n-1}\times \su$ because $T\cong (S^1)^{n-1}$. Therefore by Corollary \ref{ex 2}, the bundle gerbe (\ref{eqn}) is stably isomorphic to  $$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right) .$$
	Let us understand what this bundle gerbe looks like fibrewise. Since the projection map $\R^{n-1}\times \su \to T\times \su$ is the identity on the $\su$ factor, we have $$\left(\R^{n-1}\times \su\right)^{[2]} \cong \left(\R^{n-1}\right)^{[2]}\times \su$$ where the fibre product $\left(\R^{n-1}\right)^{[2]}$ is taken with respect to the projection $\R^{n-1}\to \left(S^1\right)^{n-1}$ given by $(x_1, ..., x_{n-1})\mapsto ([x_1], ..., [x_{n-1}])$. Let $(x, y, gT)\in \left(\R^{n-1}\right)^{[2]}\times \su$. Write $x$ and $y$ as $n$-tuples $(x_1, ..., x_n)$ and $(y_1, ..., y_n)$ respectively, whose coordinates sum to zero. Then  \begin{align}
	\left(\Motimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (J_1\cup p_1)_{(x_1, y_1, gT)} \otimes \cdots \otimes (J_n\cup p_n)_{(x_n, y_n, gT)}  \nonumber  \\
	&= (J_1)_{gT}^{d(x_1, y_1)}\otimes \cdots \otimes (J_n)_{gT}^{d(x_n, y_n)}.\label{Jifibres}
	\end{align}
	% Define for each $i=1, ..., n$ the map $p_i: \R^{n-1}\to \R$ defined by $p_i(x^1, ..., x^n)= x^i$ where again we identify $\R^{n-1}$ with the the subset of $\R^n$ whose coordinates sum to zero. Then \begin{align*}
	%\left(\bigotimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (L_1)_{gT}
	% \end{align*}
	
	The following proposition follows immediately from Propositions \ref{equivariantbundlegerbeproduct} and \ref{cupprodisequivariant}.
	\begin{proposition}
		The bundle gerbe $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ defined above is $SU(n)$-equivariant. 
	\end{proposition}
	\subsection{Geometry of the flag manifold}
	
	\indent \indent Let $F_n$ be the manifold whose points are sets $\{W_1, ..., W_n\}$ of mutually orthogonal one-dimensional subspaces of $\C^n$ ($F_n$ is the \textit{flag manifold} of $\C^n$). Let $e_1, ..., e_n$ be the standard basis vectors of $\C^n$ and define the \textit{standard element} $e$ of $F_n$ by $e := \{E_1:=\text{span}(e_1), ...,E_n:=\text{span}(e_n)\}$. Consider the action of $U(n)$ on $F_n$ defined by multiplication $$g\cdot \{W_1, ..., W_n\} := \{g W_1, ..., g W_n\}.$$ Let $\{W_1, ..., W_n\}, \{V_1, ..., V_n\}\in F_n$ and choose basis elements of $w_i$ and $v_i$ for each $W_i$ and $V_i$ respectively so that $\{w_i\}_{i=1}^n$ and $\{v_i\}_{i=1}^n$ are orthonormal basis of $\C^n$. Recall from elementary algebra that the transition matrix mapping $\{w_i\}$ onto $\{v_i\}$ is unitary. Therefore this (smooth) action of $U(n)$ on $F_n$ is transitive. Moreover, the isotropy group of $e$ is the torus $T$. So by Theorem \ref{theorem} $$U(n)/T \cong F_n.$$
	Any element $\{W_i\}_{i=1}^n \in F_n$ can be identified with a set of orthogonal projections $\{P_i\}_{i=1}^n$ for $P_i:\C^n\to W_i$.  By orthogonality, $P_iP_j = 0$ if $i\neq j$ and $\sum_{i=1}^n P_i = 1$. Therefore elements of $U(n)/T \times T$ can be identified with pairs $(P, t)$ where $P = (P_1, ..., P_n)$ are orthogonal projections and $t = \text{diag}(p_1(t), ..., p_n(t))$. The $p_i(t)$ can be thought of as the eigenvalues of a unitary matrix $g$, with $P_i$ being the orthogonal projections onto the $p_i(t)$-eigenspace. By requiring $p_1(t)\cdots p_n(t) = 1$, pairs $(P, t)$ can be identified with $\su\times T$.  With this description in mind, the Weyl map $p: SU(n)/T\times T\to SU(n)$ becomes \begin{align} \label{weylmapdescription} (P, t)\mapsto \sum_{i}p_i(t)P_i \end{align} To see this, consider the identification \begin{gather*}
	T\times \su \to T\times F_n\\
	(t, gT) \mapsto (t, gE_1g^{-1}, ..., gE_ng^{-1}).
	\end{gather*} Then $$p(t, gT) = gtg^{-1} = g\left(\textstyle \sum_{i=1}^n p_i(t)E_i\right)g^{-1} =  \textstyle \sum_{i=1}^n p_i(t) \left(gE_ig^{-1}\right)$$ so $p(t, gE_1g^{-1},..., gE_ng^{-1}) =   \textstyle \sum_{i=1}^n t_i \left(gE_ig^{-1}\right)$, giving us the description of the Weyl map on $T\times F_n$ above. 
	\subsection{Connective structure on the cup product bundle gerbe} 
	In this section we aim to compute blah blah blah  in three steps. Herein we shall refer to a bundle gerbes $ \left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i\in \{1, ..., n\}$ as the \textit{$i$-th cup product bundle gerbe}.
	% Recall the line bundle $\widetilde{J}_i\to \su$ with $\widetilde{J}_i := SU(n)\times \C /\sim_{\widetilde{p}_i}$ defined in Example \ref{ex 1}. 
	\begin{proposition}\label{curvaturetwoform}
		For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla^{{J}_i}$ on ${J}_i\to \su$ with curvature $F_{\nabla_{{J}_i}} = \textup{tr}(P_idP_idP_i)$ for $P_i:\su\times \C^n\to J_i $ orthogonal projection which is point-wise a map $P_i(gT): \{gT\} \times \C^n\to (J_i)_{gT} \subset \{gT\}\times \C^n$. 
	\end{proposition}
	
	%\begin{proposition}
	%	For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla_i$ on $J_i\to T\times \su$ with curvature $$F_{\nabla_i} = \text{tr}(P_idP_idP_i)$$ for $P_i:\su\times \C\to J_i$ orthogonal projection. 
	%\end{proposition}
	\begin{proof} To show this, we will utilise Example \ref{linebundleconnection}. To do so, let us first understand ${J}_i$ as a subbundle of a trivial bundle of rank $n$. Now, ${J}_i$ is a subbundle of the $SU(n)$-homogeneous line bundle $\frac{SU(n)\times \C^n}{T}\to \su$. The latter is isomorphic to the trivial bundle $\su \times \C^n \to \su$ by Theorem \ref{thrmbundles}. Therefore by Example \ref{linebundlecurvature} projection of the trivial connection gives us a connection $\nabla_{{J}_i}:= P_i(d)$ on ${J}_i\to \su$ with curvature two form $F_{\nabla_{{J}_i}} = \text{tr}(P_idP_idP_i)$. \end{proof}
	
	\begin{remark}\label{remark curvatureofJ} 
		Recall that (abusing notation) we have the line bundle $J_i \to T\times \su$ defined by pulling back $J_i\to \su$ along $T\times \su\to \su$. Using that there is an induced pullback connection on $J_i\to T\times \su$, it is not difficult to show by the previous proposition that the pullback connection on $J_i\to T\times \su$ has curvature $\text{tr}(P_idP_idP_i)$ for $P_i: \su \times T\times \C^n \to J_i$ orthogonal projection. Just as we abuse notation with the line bundles $J_i$, we abuse notation and write the curvatures of the connections on these respective line bundles as $\text{tr}(P_idP_idP_i)$ despite the projections being defined on different spaces. 
	\end{remark}
	
	%
	%\begin{corollary}\label{curvatureofJ} 
	%	For each $i=1, ..., n$ there is a canonical line bundle connection $\nabla^{J_i}$ on $J_i\to T\times \su$ with curvature $$F_{\nabla^{J_i}} = \textup{tr}(P_idP_idP_i) $$ for $P_i:T\times \su \times \C \to J_i$ orthogonal projection.
	%\end{corollary}
	%\begin{proof}
	%Recall that $J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1} \widetilde{J}_i$ for $\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su \to \su$ projection. So we can pullback the connection $\nabla^{\widetilde{J}_i}$ on $\widetilde{J}_i\to \su$ defined above to obtain the connection $$\nabla^{J_i}:= \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}\nabla^{\widetilde{J}_i}$$ on $J_i\to T\times \su$. This connection has curvature two form $F_{\nabla^{J_i}} = \pi_{\smath{ \dfrac{SU(n)}{T} } }^{*} F_{\nabla^{\widetilde{J}_i}}$. Pulling back the curvature two form $F_{\nabla^{\widetilde{J}_i}}$ from Proposition \ref{curvaturetwoform} is equivalent to pulling back the orthogonal projections $\su \times \C\to \widetilde{J}_i$ in its definition along $\su\times T \times \C\to \su\times \C$, giving us the result. {\textcolor{red}{is this right?}} 
	%\end{proof}
	
	
	\begin{proposition}\label{existsconnectiononcup} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Let $f:M\to S^1$ be a smooth map. For each $k\in \Z$ define the projection $$\pi_k: \{k\}\times f^{-1}(\R)\to M.$$Then on the cup product bundle gerbe $\left(P\cup f, f^{-1}(\R), M\right)$ there is a bundle gerbe connection $\nabla_{P\cup f}$ with curvature two-form $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ on connected components of $\Z\times f^{-1}(\R) \cong f^{-1}(\R)^{[2]}$.  
	\end{proposition}
	\begin{proof}
		Over $\{k\}\times f^{-1}(\R)$, $P\cup f = \pi_k^{-1}(P)^k$, so $\pi_k^{-1}(\nabla)^k$ defines a connection on connected components $\{k\}\times f^{-1}(\R)$ of $\Z\times f^{-1}(\R)$, hence defines a global connection $\nabla_{P\cup f}$ on $P\cup f \to \Z\times f^{-1}(\R)$. This is a bundle gerbe connection since, for $(n, t_1, t_2, t_3)\in f^{-1}(\R)^{[2]}$ and $m$ the bundle gerbe multiplication on $P\cup f$, $$m\left((P_n)^{t_1-t_3}\otimes (P_n)^{t_1-t_2}\right) = (P_n)^{t_1-t_3}$$ implies $$m(\nabla^{t_1-t_2}\otimes 1 + 1\otimes \nabla^{t_1-t_2}) = \nabla^{t_1-t_3}, $$ which is precisely what it means for $\nabla_{P\cup f}$ to be a bundle gerbe connection in this instance. It then follows immediately by Proposition \ref{constructingconnections} that $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ for all $k\in \Z$.
	\end{proof}
	\begin{example}\label{connectiononJ}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i= 1, ..., n$. For each $k\in \Z$ let $$\pi_{k,i}: \{k\}\times p_i^{-1}(\R)\to T\times \su $$ be projection and $\nabla_{J_i}$ a connection on $J_i\to T\times \su$. Then by the previous proposition, there is a bundle gerbe connection $\nabla_{J_i\cup p_i}$ on the $i$-th cup product bundle gerbe with two-curvature $$ F_{\nabla_{J_i\cup p_i}}\big |_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_{k,i}^{*}F_{\nabla_{J_i}}.$$
	\end{example}
	
	
	%\begin{proposition}\label{connectiononJ}
	%Consider the $i$-th cup product bundle gerbe for $i\in \{1, ..., n\}$.  Let $k\in \Z$, and define the projection $$\pi_{k}: \{k\}\times p_i^{-1}(\R) \to \su $$ onto the $\su$ element of $p_i^{-1}(\R)$. There is a bundle gerbe connection $\nabla^{\cup_i}$ on the $i$-th cup product bundle gerbe with curvature two-form $$F_{\nabla^{\cup_i}} \big\rvert_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_k^{-1}\left(F_{\nabla^{\widetilde{J}_i}}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)\cong p_i^{-1}(\R)^{[2]}$.
	%\end{proposition}
	%
	%\begin{proof} Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ as in Remark \ref{isocup}. To define a line bundle connection on $J_i\cup p_i\to \Z\times \left(\widetilde{p}_i\right)^{-1}(\R) \times \su$ it suffices to define a connection on connected components $U_k:= \{k\}\times p_i^{-1}(\R)$ for $k\in \Z$. Recall $\widetilde{J}_i\to \su$ has line bundle connection $\nabla^{\widetilde{J}_i}$. Hence $\nabla^{\widetilde{J}_i^k}$ is a connection on $\widetilde{J_i}^k \to \su$. So $\pi_k^{-1}\nabla^{\widetilde{J}_i}$ defines a connection on $\pi_k^{-1}\widetilde{J}_i^k \cong J_i\cup p_i \big\rvert_{\{k\}\times p_i^{-1}(\R)}$ This is a bundle gerbe connection because $\nabla^{\widetilde{J}_i}$ is. It follows immediately that the two curvature of the connection $\pi_k^{-1}\left(\nabla^{\widetilde{J}_i^k}\right)$ is $k\cdot \pi_k^{-1}(F_{\nabla^{\widetilde{J}_i}})$ by Proposition \ref{constructingconnections}. \end{proof}
	\begin{remark}
		By Proposition \ref{tensorproductconnection} and Proposition \ref{constructingconnections}, there is a bundle gerbe connection $\nabla^{\otimes \cup}$ on  $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ with curvature two form $$F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{*}\left(F_{\nabla^{{J}_i}}\right)  $$ over connected sets $\{(k_1, ..., k_{n-1})\}\times \R^{n-1}\times \su \subset \Z^{n-1}\times \R^{n-1}\times \su \cong \left(\R^{n-1}\times \su\right)^{[2]}$ with $k_n := -k_1 - \cdots - k_{n-1}$. By Remark \ref{remark curvatureofJ} this can be written as $$ F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{-1}\left(\text{tr}(P_idP_idP_i)\right)$$ for $P_i: T\times \su \times \C^n \to {J}_i$ orthogonal projection. 
	\end{remark}
	%\text{}\\ 
	%of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$
	
	
	
	
	
	\begin{proposition} \label{curvaturetheorem1} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Consider the cup product bundle gerbe $(P\cup f, f^{-1}(\R), M)$ defined for $f:M\to S^1$ a smooth map. Let $\pi:f^{-1}(\R)\to M$ be the surjective submersion in this bundle gerbe and $\nabla_{P\cup f}$ the bundle gerbe connection from Proposition \ref{existsconnectiononcup}. Define a two-form $h$ on $f^{-1}(\R)$ by $$h(m, x) = x \cdot \pi^*F_\nabla. $$ Then 
		\begin{enumerate}[(1),font=\upshape]
			\item the two form $h$ satisfies $\delta(h) = F_{\nabla_{P\cup f}}$, so $h$ is a curving for the bundle gerbe connection $\nabla_{P\cup f}$;
			\item the three-curvature $\mu \in \Omega^3(M)$ of the bundle gerbe connection $\nabla_{P\cup f}$ is given by $$\mu =  \frac{1}{2\pi}\, f^{*}(d\theta) \wedge F_{\nabla} $$ for $\theta \in (0,2\pi)$ the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class of $(P\cup f, f^{-1}(\R), M)$ is 
			$$\frac{-i}{4\pi^2}\, f^{*}(d\theta) \wedge F_{\nabla}.$$ 
		\end{enumerate}
	\end{proposition}
	
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	
	\begin{proof} Let us first compute $\delta(h)$. Now, for $(m, x, x') \in f^{-1}(\R)^{[2]}$
		
		\begin{align*}
		\delta(h)\big\rvert_{(m, x, x')} &= \pi_1^{-1} h \big \rvert_{(m, x, x')}   - \pi_2^{-1}h\big\rvert_{(m, x, x')} \\ 
		&=  h\big\rvert_{(m, x')}\circ d\pi_1-  h\big\rvert_{(m, x)}\circ d\pi_2
		\end{align*}
		By noting that $T\Z = 0$ and $f^{-1}(\R)^{[2]} \cong \Z \times f^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla}\big\rvert_{(m, x')} = \pi^{-1}F_{\nabla}\big\rvert_{(m, x)}$. Therefore at a point $(m, x, x')\in f^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
		\delta(h) &= k \cdot \pi^{-1}F_{\nabla}\circ d\pi_1 \big |_{\{k\}\times f^{-1}(\R)}\\ 
		&= k\cdot (\pi\circ\pi_1 |_{\{k\}\times f^{-1}(\R)})^{-1}F_{\nabla}\\
		&= k\cdot \pi_k^* F_{\nabla}\\
		&= F_{\nabla_{P\cup f}}\big |_{\{k\}\times f^{-1}(\R)}.
		\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu\in \Omega^3\left(M\right)$ is defined implicitly by $$dh = \pi^{*}\mu.$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (f\circ \pi)^{*}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
		dh&= d\left(x \cdot \pi^{*}F_\nabla\right)\\
		&= dx \wedge \pi^{*}F_{\nabla}\\
		&= \frac{1}{2\pi} \, \pi^{*}\left(f^{*}(d\theta)\wedge F_{\nabla}\right). 
		\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	
	\begin{example}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ with surjective submersion $\pi_i: p_i^{-1}(\R)\to T\times \su$  and connection and curvature $\nabla^{\cup_i}$, $F_{\nabla^{\cup_i}}$. By the previous proposition, this bundle gerbe has curving $h_i \in \Omega^2(p_i^{-1}(\R))$ given by $$h_i(t, gT, x) = x\cdot \pi_i^* F_{\nabla^{J_i}}$$ and three-curvature $\mu_i\in \Omega^3(T\times \su)$ given by $$\mu_i = \frac{1}{2\pi}\, p_i^*(d\theta) \wedge F_{\nabla^{J_i}}.$$ Moreover, the Dixmier-Douady class of the $i$-th cup product bundle gerbe is $$-\frac{i}{2\pi^2}\, p_i^*(d\theta)\wedge F_{\nabla^{J_i}}. $$
	\end{example}
	
	
	%
	%
	%\begin{proposition}
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	%	\end{proposition}
	%\begin{proof} Let us first compute $\delta(h_i)$. Now, for $(t, gT, x, x') \in p_i^{-1}(\R)^{[2]}$ \begin{align*}
	%\delta(h_i)\big\rvert_{(t, gT, x, x')} &= \pi_1^{-1} h_i \big \rvert_{(t, gT, x, x')}   - \pi_2^{-1}h_i \big\rvert_{(t, gT, x, x')} \\ 
	%&=  h_i\big\rvert_{(t, gT, x')}\circ d\pi_1-  h_i\big\rvert_{(t, gT, x)}\circ d\pi_2
	%\end{align*}
	%By noting that $T\Z = 0$ and $p_i^{-1}(\R)^{[2]} \cong \Z \times p_i^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x')} = \pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x)}$. Therefore at a point $(t, gT, x, x')\in p_i^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
	%\delta(h_i) &= k \cdot \pi^{-1}F_{\nabla^{J_i}}\circ d\pi_1\\ 
	%&= k\cdot (\pi\circ\pi_1)^{-1}F_{\nabla^{J_i}}\\
	%&= k\cdot \left(\pi_{\smath{ \dfrac{SU(n)}{T} } }\circ \pi \circ \pi_1\right)^{-1} F_{\nabla^{\widetilde{J}_i}}\\
	%&= k \cdot \pi_k^{-1}F_{\nabla^{\widetilde{J}_i}}\\
	%&= F_{\nabla^{\cup_i}}.
	%\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu_i \in \Omega^3\left(T\times \su\right)$ is defined implicitly by $$dh_i = \pi^{-1}(\mu_i).$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (p_i\circ \pi)^{-1}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
	%dh_i &= d\left(x \cdot \pi^{-1}\left(F_{\nabla^{J_i}}\right)\right)\\
	%&= dx \wedge \pi^{-1}\left(F_{\nabla^{J_i}}\right)\\
	%&= \pi^{-1}\left(\textstyle \frac{1}{2\pi} p_i^{-1}(d\theta)\wedge F_{\nabla^{J_i}}\right). 
	%\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	% Let us first construct the connection on the cup product bundle gerbe. Consider a connected open subset $U\subseteq f^{-1}(\R)^{[2]}$. Recall that $f^{-1}(\R)^{[2]}$ consists of triples $(m, t_1, t_2) \in M\times \R^2$ satisfying $f(m) = [t_1] = [t_2]$. The difference map $d:\R^{[2]}\to \Z$ is continuous and therefore constant on connected components. Therefore for all $(m, t_1, t_2) \in U$, $t_1-t_2 = k$ for some fixed integer $k$. {\textcolor{red}{need to think about connectedness of product I'm getting confused}} Therefore $$(P\cup f)|_U = P^k|_U.$$ Let $\nabla$ be a connection on $P\to M$. Then $\nabla^k$ is a connection on $(P\cup f)|_{U_k}$. Since we can do this for all connected subsetes $U_k$ of $f^{-1}(\R)^{[2]}$, we have a connection $\nabla^{P\cup f}$ on all of $P\cup f$. To see that this is a bundle gerbe connection, recall that bundle gerbe multiplication on $P\cup f$ is given by $$(P_m)^{t_2-t_3} \otimes (P_m)^{t_1-t_2} = (P_m)^{t_1-t_3}.$$ Certainly $$\nabla^{t_1-t_2}\otimes \nabla^{t_1-t_2} = \nabla^{t_1-t_3}$$ so this connection respects the bundle gerbe multiplication.\text{}\\ \text{}\\ 
	%\indent Let $\{U_\alpha\}_{\alpha \in I}$ be an open cover of $M$ such that for each $U_\alpha$ there exists a non-vanishing section $s_\alpha: U_\alpha\to P$. Then there exists connection one forms $A_\alpha \in \Omega^1(U_\alpha)$ for which the connection $\nabla$ on $P\to M$ satisfies $$\nabla s_\alpha = A_\alpha s_\alpha.$$ Let us now find an expression for the connection one forms on $P\cup f\to f^{-1}(\R)^{[2]}$. It suffices to find the connection one forms corresponding to the connection $\nabla^k$ on $P^k|_{U_k}\to {U_k}$ by the above discussion. It is easy to verify that on $P^k|_{U_k}\to {U_k}$ the connection one forms are $$kA_\alpha \in \Omega^1(U_k\cap U_\alpha).$$ Therefore locally $F_{\nabla^k} = kdA_\alpha$, and since $F_{\nabla^{P\cup f}|_{U_k}} = F_{\nabla^k}$, this gives us a local expression for $F_{\nabla^{P\cup f}}$. Next, define $f\in \Omega^2(f^{-1}(\R))$ by $f(m, x) = x\cdot \pi^* F_\nabla$ where $\pi:f^{-1}(\R) \to M$ is the projection map. It can be verified that $f$ is a curving for $kA_\alpha$, that is, (locally) $\delta(f) = kdA_\alpha$ (where we are really pulling the latter two form back by the projection $f^{-1}(\R)^{[2]}\to M$). We can now compute the three-curvature. Now,  \begin{align*}
	%df = d(x\pi^*F_\nabla) = dx\wedge \pi^*F_\nabla = \pi^*(f^* d\theta \wedge F_\nabla)
	%\end{align*} 
	%{\textcolor{red}{really confused with this entire thing. struggling to write this concisely without using all of the pullbacks hidden in here. Also don't understand why we have $d\theta$ here when we actually want it to be $\lambda_k^*d\theta$. }}
	\begin{corollary}\label{corollary data on cup prod} 
		Consider the tensor product of the cup product bundle gerbes$$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$$ with connection $\nabla^{\otimes \cup}$ and curvature $F_{\nabla^{\otimes \cup}}$. Let $h_i$ and $\mu_i$ be the curving and three curvature respectively of the $i$-th cup product bundle gerbe with connection $\nabla^{\cup_i}$. Let $P_i$ be orthogonal projection $T\times \su\times \C^n\to J_i$. Then \begin{enumerate}[(1),font=\upshape]
			\item the two form $$h := \sum_{i=1}^n h_i$$ on $\R^{n-1}\times \su$ satisfies $\delta(h) = F_{\nabla^{\otimes \cup}}$, ie. $h$ is a curving for the connection $\nabla^{\otimes \cup}$;
			\item the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1} dp_i\wedge \textup{tr}(P_idP_idP_i)$$for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class is $$\frac{-i}{4\pi^2}\sum_{i=1}^n p_i^{-1} d p_i\wedge \textup{tr}(P_idP_idP_i).$$ 
		\end{enumerate}
	\end{corollary}
	\begin{proof}  By Theorem \ref{curvaturetheorem1}, the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi}\sum_{i=1}^n p_i^{-1}(d\theta)\wedge \text{tr}(P_idP_idP_i)$$ and the Dixmier-Douady class is $\frac{1}{2\pi i } \mu$. Using the coordinates $\theta = -i\log$ on $S^1$, we find that the pullback of $d\theta$ by $p_i: T\times \su \to S^1$ is $$p_i^{-1}(d\theta) = -i\frac{dp_i}{p_i}.$$ Therefore the three curvature of $\nabla^{\otimes \cup}$ can be rewritten as $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1}dp_i \text{tr}(P_idP_idP_i),$$ and similarly for the Dixmier-Douady class.\end{proof}
	
	%I am proving the following proposition. 
	%\begin{proposition}\label{connectiononJ}
	%	Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ for each $i=1, ..., n$. Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ and denote the surjective submersion $\Z\times p_i^{-1}(\R)\to T\times \su$ by $\pi$. Then for each $i=1, ..., n$, there is a bundle gerbe connection $\nabla^{J_i\cup p_i}$ on $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ with curvature two-form given by $$F_{\nabla^{J^i\cup p_i}} \big\rvert_{\{n\}\times p_i^{-1}(\R)} = n \cdot \pi^{-1}\left(F_{\nabla_i}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)$.
	%\end{proposition}
	
%	\textit{Proof}. Consider a connected component $U_n:= \{n\}\times p_i^{-1}(\R)$ of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$


==> chapter3/CHP3__Kim_Becker_s_conflicted_copy_2019-03-24_.tex <==
%!TEX root = ../thesis.tex
\chapter{The basic bundle gerbe\label{ch:three}}

\indent \indent Equipped with the foundational knowledge from the previous chapter, we can define the two bundle gerbes central to our research: the so called \textit{basic bundle gerbe} and the \textit{cup product bundle gerbe}. We dedicate this chapter to defining the former bundle gerbe and computing its connective data. The basic bundle gerbe can be defined in full generality over a base space $G$ for $G$ a group of unitary operators. In this work, we take $G = SU(n)$ and denote the basic bundle gerbe by $\basicbg$. As we shall see, the basic bundle gerbe is most naturally defined using line bundles. This was indeed our motivation to define bundle gerbes using line bundles rather than principal $U(1)$-bundles (Remark \ref{principalbundle}). We proceed by considering the pullback of the basic bundle gerbe along the Weyl map $$p:T\times \su \to SU(n),$$ which we denote by $\pullbackbasicbg$. we consider an equivalent description of the pullback of the basic bundle gerbe via the Weyl map using the Lie theory from Chapter 1. This description will be crucial to defining a stable isomorphism of these bundle gerbes in the next chapter. Using the results of \cite{53UNITARY}, we present the connective data associated to this bundle gerbe, and the data associated to its pullback by $p$. 


As we will see, defining both the cup product bundle gerbe over $T\times \su$ and the basic bundle gerbe is a non-trivial task. Consequently, one begins to appreciate the complexities of this field that could not be conveyed in the introductory theory. 

After introducing these bundle gerbes, we will compute their geometric data in preparation for the proceeding chapter.


The cup product construction allows us to define a bundle gerbe over $M$ given a line bundle $L\to M$ and a map $f:M\to U(1)$. In particular, we will consider the `$i$-th' cup product bundle gerbe over $T\times \su$ constructed from a line bundle $J_i\to T\times \su$ and a homomorphism $p_i: T\times \su\to U(1)$ for $T$ a maximal torus of $SU(n)$ and $i= 1, ..., n$. Finally, we form the tensor product of these $n$ bundle gerbes to form a single bundle gerbe over $T\times \su$, which, for lack of a better name, we will also refer to as the cup product bundle gerbe (over $T\times \su$). While we require a line bundle and smooth map to define the cup product bundle gerbe, the basic bundle gerbe, in contrast, is determined by its base space $G$ for $G$ a group of unitary operators. In this work, we take $G = SU(n)$. After defining the basic bundle gerbe, we will consider its pullback along the Weyl map $p:T\times \su \to SU(n)$. As we will see, defining both the cup product bundle gerbe over $T\times \su$ and the basic bundle gerbe is a non-trivial task. Consequently, one begins to appreciate the complexities of this field that could not be conveyed in the introductory theory. After introducing these bundle gerbes, we will compute their geometric data in preparation for the proceeding chapter.\\
\indent \indent We begin this chapter by defining a cup product bundle gerbe over arbitrary $M$.  In this general setting, we calculate the bundle gerbe's connective structure, three curvature and Dixmier-Douady class, before applying these results to the $i$-th cup product bundle gerbe. We conclude the first section of this chapter by computing the geometric data of the cup product bundle gerbe over $T\times \su$. In the second half of this chapter we proceed in a similar manner to define the basic bundle gerbe over $SU(n)$ and compute its connective data. As we will see, this data for the basic bundle gerbe is most naturally presented in terms of orthogonal projections. It is, however, a non-trivial exercise to translate the connective data from the cup product bundle gerbe to the language of projections. To do so, we dedicate a short section to the theory of flag manifolds. Finally, we consider an equivalent description of the pullback of the basic bundle gerbe via the Weyl map using the Lie theory from Chapter 1. This description will be crucial to defining a stable isomorphism of these bundle gerbes in the next chapter.\\ 
 \indent \indent The calculations in this chapter demonstrate many of the standard computational techniques used in this field. Furthermore, this section provides concrete examples of the geometric objects and constructions introduced in the previous chapter. These curvature calculations to come allow us to better understand these bundle gerbes in the first instance, and will also be essential to finding a stable isomorphism between these bundle gerbes. 

%After defining the basic bundle gerbe over $SU(n)$ and considering its geometry, we draw our attention to the pull back of the basic bundle gerbe along the Weyl map $p:T\times \su \to SU(n)$. The resulting bundle gerbe is defined over the same space as the cup product bundle gerbe, namely $T\times \su$. \\ 
%
% The construction of the cup product bundle gerbe will be discussed at the beginning of this chapter. After this, we will study the geometry of the cup product bundle gerbe, and apply these result to our cup product bundle gerbe of interest. 


\section{Definition} 
We define the basic bundle gerbe over $SU(n)$ as follows, using \cite{53UNITARY}. {\textcolor{red}{more intro}} 


Let $Z := U(1)\backslash \{1\}$ and denote the set of eigenvalues of an operator $g\in SU(n)$ by spec$(g)$. Define $$Y:= \{(z, g) \in Z\times SU(n) \ | \ z\notin \text{spec}(g)\}.$$ Let $\pi: Y\to SU(n)$ be projection onto the second factor. This will be the surjective submersion of the basic bundle gerbe over $SU(n)$. Note that $$Y^{[p]} = \{(z_1, ..., z_p, g) \in Z^p \times SU(n) \  | \ z_1, ..., z_p \notin \text{spec}(g) \}.$$  \\ \text{}\\
\indent \indent It remains to define the line bundle $\Pbasic \to Y^{[2]}$. We do so by defining $\Pbasic$ over the connected components of $Y^{[2]}$, which can be described explicitly using an ordering on $Z$. To see this, first note that the natural ordering of elements in $(0, 2\pi)$ endows $Z$ with an ordering. Explicitly, we can define a map $\text{arg}: Z \to (0, 2\pi)$ satisfying $\text{exp}(i\text{arg}(s)) = s$ for all $s\in Z$. Then given $z_1, z_2 \in Z$, define $z_1 < z_2$ if $\text{arg}(z_1) < \text{arg}(z_2)$.  Say that $\lambda \in Z$ is \textit{between} $z_1$ and $z_2$ if $z_1 < \lambda < z_2$ or $z_2 < \lambda < z_1$ (equivalently, $\lambda$ is between $z_1$ and $z_2$ if $\lambda$ is in the connected component of $U(1)\backslash\{z_1, z_2\}$ not containing $\{1\}$). Call a triple $(z_1, z_2, g)\in Y^{[2]}$ \textit{positive} if there exist eigenvalues of $g$ between $z_1 > z_2$, \textit{null} if there are no eigenvalues of $g$ between $z_1$ and $z_2$, and \textit{negative} if there exist eigenvalues of $g$ between $z_1<z_2$. Note that $(z_1, z_2, g)$ is positive if and only if $(z_2, z_1, g)$ is negative. Denote the connected subsets of $Y^{[2]}$ consisting of positive, null, and negative triplets by $Y^{[2]}_+, Y^{[2]}_0$ and $Y^{[2]}_{-}$ respectively. To be completely explicit, \begin{align*}
Y_+^{[2]} &= \{(z_1, z_2, g)\in Y^{[2]} \ | \ \exists \ \lambda \in \text{spec}(g) \text{ with } z_1>\lambda > z_2 \} \\
Y_0^{[2]} &= \{(z_1, z_2, g)\in Y^{[2]} \ | \ \nexists \ \lambda \in \text{spec}(g) \text{ with } z_2>\lambda > z_1 \text{ or } z_1>\lambda > z_2  \}\\
Y_-^{[2]} &= \{(z_1, z_2, g)\in Y^{[2]} \ | \ \exists \ \lambda \in \text{spec}(g) \text{ with } z_2>\lambda > z_1 \}.
\end{align*} 
Next, for any $(g, \lambda) \in SU(n)\times Z$, define $E_{(g, \lambda)}$ to be the $\lambda$-eigenspace of $g$. Define a vector bundle $L\to Y^{[2]}_{+}$ fibrewise by $$L_{(z_1, z_2, g)} = \Moplus_{z_1>\lambda > z_2} E_{(g, \lambda)}.$$ 
Note that $L_{(z_1, z_2, g)}$ has finite dimension as a finite sum of finite-dimensional spaces, therefore we may define $$(\Pbasic)_{(z_1, z_2, g)} = \begin{cases} \text{det}(L_{(z_1, z_2, g)}) &\text{if } (z_1, z_2, g)\in Y^{[2]}_+\\ 
\C&\text{if } (z_1, z_2, g)\in Y^{[2]}_0 \\
\text{det}(L_{(z_2, z_1, g)})^* & \text{if } (z_1, z_2, g) \in Y^{[2]}_{-}. \end{cases} $$
It follows that $\Pbasic \to Y^{[2]}$ is a smooth locally trivial hermitian line bundle by \cite{53UNITARY}. \\
\indent \indent Finally, we define a multiplication operation $m: \pi_3^{-1}(\Pbasic) \otimes \pi_1^{-1}(\Pbasic) \to \pi_2^{-1}(\Pbasic)$ that will endow $\basicbg$ with bundle gerbe structure. Let $(z_1, z_2, z_3, g) \in Y^{[3]}$ with $z_1>z_2>z_3$. Assume there are eigenvalues of $g$ between $z_1$ and $z_2$ and also between $z_2$ and $z_3$. Clearly $$\Moplus_{z_1 >\lambda > z_2 } E_{(g, \lambda)} \ \oplus \Moplus_{z_2>\lambda > z_3 } E_{(g, \lambda)} = \Moplus_{z_1 >\lambda > z_3 } E_{(g, \lambda)} $$ and so for this choice of $(z_1, z_2, z_3, g)\in Y^{[3]}$ the fibres of $L$ satisfy \begin{align}\label{eqn3} L_{(z_1, z_2, g)}\oplus L_{(z_2, z_3, g)} = L_{(z_1, z_3, g)}.\end{align} Recall that the wedge product defines a canonical isomorphism $\text{det}(V)\otimes \text{det}(W)\to \text{det}(V\oplus W)$ for vector spaces $V$ and $W$. Therefore in this case, the wedge product defines an isomorphism (and indeed, a bundle gerbe multiplication) $$(\Pbasic)_{(z_1, z_2, g)}\otimes (\Pbasic)_{(z_2, z_3, g)}= (\Pbasic)_{(z_1, z_2, g)}.$$ Associativity of this multiplication follows by associativity of the wedge product, making $\basicbg$ into a bundle gerbe.
\begin{definition}
	Call the bundle gerbe $\basicbg$ constructed above the \textit{basic bundle gerbe}. 
\end{definition}
Before moving on to discuss the pullback of the basic bundle gerbe by the Weyl map, let us consider one property of the basic bundle gerbe critical to our later work. Note that $SU(n)$ is a compact Lie group which acts on itself by conjugation. It is then natural to ask if the basic bundle gerbe is $SU(n)$-equivariant. This is indeed the case, leading us to our next proposition.
\begin{proposition}\label{proposition basic bg is equivariant} 
	The basic bundle gerbe $\basicbg$ is an $SU(n)$-equivariant bundle gerbe. 
\end{proposition}
\begin{proof} We provide an outline of this proof and refer the reader to \cite{53UNITARY} for further details. First, we see that the conjugation action of $SU(n)$ on itself lifts to an action on $Y$ defined by $g \cdot(z, s) :=
(z, gsg^{-1})$. This is of course well defined since $\text{spec}(s) = \text{spec}(gsg^{-1})$. Clearly $\pi:Y\to M$ is $SU(n)$-equivariant, so we need only verify that $\Pbasic \to Y^{[2]}$ is an $SU(n)$-equivariant line bundle. We show this is true for the restriction of $\Pbasic\to Y^{[2]}$ to $Y^{[2]}_+$ and claim the other cases proceed similarly. Let $(z_1, z_2, g) \in Y_+^{[2]}$ and $h\in SU(n)$. Consider an eigenvector $v\in L_{(z_1, z_2, g)}$ with eigenvalue $\lambda$. Then $hv$ is an eigenvector of $hgh^{-1}$ with eigenvalue $\lambda$, so multiplication by $h$ defines an action $L_{(z_1, z_2, g)}\to L_{(z_1, z_2, hgh^{-1})}$. Since $\Pbasic|_{Y_+^{[2]}} = \text{det}(L)$, there is an induced action on $\Pbasic|_{Y_+^{[2]}}$ (which is linear on fibres). Lastly, the projection $\Pbasic|_{Y_+^{[2]}}\to Y_+^{[2]}$ is $SU(n)$-equivariant, so $\Pbasic|_{Y_+^{[2]}}\to Y_+^{[2]}$ is an $SU(n)$-equivariant line bundle.
%
%Recall that $\Pbasic\big\rvert_{Y_+^{[2]}} := \text{det}\left(E\right)$ where $$E_{(z_1, z_2, g)}  = \Moplus_{z_1>\lambda>z_2} E_{(g, \lambda)}$$ for Therefore multiplication by $g\in SU(n)$ gives us an action $E_{(z_1, z_2, t)}\mapsto E_{(z_1, z_2, gtg^{-1})}$, which induces an action on $L\big\rvert_{Y_+^{[2}}$ and hence on $\Pbasic$. 
\end{proof}
\section{Pulling back by the Weyl map} 
\indent \indent In this section we consider the pullback of the basic bundle gerbe by the Weyl map and some of its equivalent descriptions. Our motivation for exploring these alternative descriptions may appear somewhat mysterious. However, we assure the reader that the results in this section will be indispensable in our final chapter. For now, let us view the computations in this section as elaborate examples of the constructions introduced in Chapter \ref{ch:two}. We encourage to the reader to skim read the results from this section, and return to this section after we apply these results in our final chapter. \\
%constructions introduced in the previous chapter.
%demonstration of commonly used techniques in this field to compute the constructions introduced in the previous chapter. 
\indent \indent \begin{example} We pullback the basic bundle gerbe by the Weyl map via the follow procedure. Consider the Weyl map $$p: T\times \su \to SU(n)$$ for $T$ a fixed maximal torus of $SU(n)$. Pulling back the surjective submersion $Y\to SU(n)$ along $p$, we obtain a surjective submersion $p^{-1}(Y)\to T\times \su$. Denote the canonical projection $p^{-1}(Y) \to Y$ by $\hat{p}$, and the induced map $p^{-1}(Y)^{[2]}\to Y^{[2]}$ by $\hat{p}^{[2]}$. Of course, $\pullbackbasicbg = (	(\hat{p}^{[2]})^{-1}(\Pbasic), p^{-1}(Y), T\times \su)$. This information is depicted in Figure \ref{fig:pullbackweyl}. 


%\begin{proposition}\label{iso1} 
%{\textcolor{green}{THIS WILL ALL BE REMOVED PROBABLY There is a bundle gerbe morphism $$\LL \frac{SU(n)\times L_T}{T}, \Su \times Y_T, \Su\times T\RR \to \LL L, Y, SU(n)\RR $$ covering the Weyl map $p: \su\times T\to SU(n)$. {\color{red}{cite 53.}} }
%\end{proposition}\textcolor{green}{
%\textit{Proof.}   {\color{red}{I've left out the G equivariance stuff put this in}} To define a bundle gerbe morphism, we require a triple of maps $\frac{SU(n)\times L_T}{T}\to L$, $\su \times Y_T\to Y$, and $ \su \times T \to SU(n)$ as in Definition \ref{bundle gerbe morphism}. Let the third map $\su \times T \to SU(n)$ be the Weyl map. Define \begin{align*}
%p_Y: \Su \times Y_T \to Y\\
%(gT, (z, t)) \mapsto (z, gtg^{-1}).
%\end{align*} Note that this is well defined since $z\notin \text{spec}(z)\cup \{1\}$ implies $z\notin \text{spec}(gtg^{-1})\cup \{1\}$. It is clear that $p_Y$ covers the Weyl map.  {\color{blue}{could insert a commutative diagram here of weyl map and this new map?}} Define a map $\frac{SU(n)\times L_T}{T}\to L$ covering the induced map $p_Y^{[2]}: \su \times Y_T^{[2]}\to Y^{[2]}$ as follows.\\
%{\textcolor{red}{consider introducing notation for $Z$} } }

\begin{figure}[h!] 
	\begin{center} 
		\begin{tikzcd}[row sep = 2em, column sep=3em]
			(\hat{p}^{[2]})^{-1}(\Pbasic) \arrow[r]  \arrow[d]		  &\Pbasic \ \  \arrow[d, shift right = .7ex]   \\
			{p}^{-1}(Y)^{[2]} \arrow[r, "\hat{p}^{[2]}"] \arrow[d, shift right=1.2ex] \arrow[d,shift left=.1ex]& Y^{[2]}  \arrow[d, shift right=1.2ex] \arrow[d,shift left=.1ex] \\
			p^{-1}(Y)  \arrow[r, "\hat{p}"] \arrow[d] &  Y \  \  \arrow[d, shift right = .7ex] \\ 
			T\times \su \arrow[r, " \ \ \ p"] & SU(n) \ \ 
			
		\end{tikzcd} 
		\caption{Pullback of $(\Pbasic, Y, SU(n))$ by $p$ }
		\label{fig:pullbackweyl} \end{center} \end{figure}

Let us better understand the spaces $p^{-1}(Y), p^{-1}(Y)^{[2]}$ and $	(\hat{p}^{[2]})^{-1}(\Pbasic)$. Recall that $Y$ is defined as the space of pairs $(z, g)\in Z\times SU(n)$ with $z\notin \text{spec}(g)$. It is not difficult to see that
\begin{align} p^{-1}(Y) &\cong \left\{(gT, z, t) \in \su \times Z \times T\ | \ z\notin \text{spec}(t)\right\}  \label{eq:test} \\ 
 p^{-1}(Y)^{[2]} &\cong \left\{(gT, t, z_1, z_2)\in \su \times T \times Z \times Z \ | \ z_1, z_2\notin \text{spec}(t)\right\}  \label{eq:test2} \\
\text{and      }\ \ \  \LL\hat{p}^{[2]}\RR^{-1}(\Pbasic) &\cong \left \{ (gT, t, z_1, z_2, v) \in p^{-1}(Y)^{[2]}\times \Pbasic \ | \ v \in (\Pbasic)_{(z_1, z_2, gtg^{-1})}\right\},   \label{eq:test3} 
\end{align} 
where we obtain Equation \ref{eq:test3} by noting that $\hat{p}^{[2]}(gT, t, z_1, z_2)=(z_1, z_2, gtg^{-1})$ under the identification in Equation  \ref{eq:test2}.\end{example} 
%\cong \left\{(gT, t, z, s) \in \su \times T \times Z\times SU(n) \ | \ z\notin \text{spec} (s), s = gtg^{-1}\right\} \nonumber 
%&
%&\cong \left\{(gT, t, z, g'T, t', z')\in p^{-1}(Y)^{2} \ | \ (gT, t) = (g'T, t')\right\} \nonumber \\&
%It follows that the induced map  Finally, we may compute the pull back of $L$ to be

%\begin{center}\includegraphics[scale=.3]{pullback3.png}\end{center}

	
\begin{remark}
	By Propositions \ref{proposition pullback equivariant bg is equivariant} and \ref{proposition basic bg is equivariant} the pullback of the basic bundle gerbe by the Weyl map is $SU(n)$-equivariant.  
\end{remark}
\indent \indent The above diffeomorphisms will allow us to define an explicit stable isomorphism between $\pullbackbasicbg$ and another bundle gerbe which we introduce now. Denote the basic bundle gerbe restricted to $T$ by $\basicbgtorus$ where $Y_T:= \{(z,g)\in Y \ | \ g\in T\}$ and $\PbasicT$ denotes the restriction of $\Pbasic$ to $Y_T^{[2]}$. Then we have the following proposition (and definition) which we present without proof. 

\begin{proposition}
Let $\PbasicT\times_T SU(n)$ be the set of equivalence classes in $\PbasicT\times SU(n)$ under the relation $$(v_1\wedge \cdots \wedge v_k, g) \sim (tv_1 \wedge \cdots \wedge tv_k, gt^{-1})$$ for all $t\in T$. Then ${\PbasicT \times_T SU(n)} \to Y_T^{[2]}\times \su$ is a line bundle with projection induced by the quotient map $SU(n)\to \su$ and the projection $\PbasicT \to Y_T^{[2]}$ restricted to $Y_T^{[2]}$. Moreover, the triple $$\left(  \PbasicT \times_T SU(n), Y_T\times \su, T\times \su \right)$$ is a bundle gerbe. 
\end{proposition}
\begin{remark}\label{remark equivariance of other bundle gerbe} 
	 It is not difficult to show that $\left(  \PbasicT \times_T SU(n), Y_T\times \su, T\times \su \right)$ bundle gerbe is $SU(n)$-equivariant with $SU(n)$ acting on each of $T\times \su$, $Y_T\times \su $, and $\PbasicT \times_T SU(n)$ by left multiplication in the $SU(n)$ component. 
%	\begin{align*} SU(n)\stackrel{}{\curvearrowright}T\times \su \ \  &\text{ by } \ \ g\cdot (t, sT) := (t, gsT)\\
%	SU(n)\stackrel{}{\curvearrowright}Y_T\times \su \ \  &\text{ by } \ \ g\cdot ((z, t), sT) := ((z,t), gsT)\\
%		\text{ and } \ \ \ \ SU(n)\stackrel{}{\curvearrowright}\PbasicT \times_T SU(n) \ \  &\text{ by } \ \ g\cdot [(v, h)] := [(v, gh)].
%	\end{align*} 
\end{remark}



%
%
% Next, let $\frac{SU(n)\times \Pbasic}{T}$ be the set of equivalence classes in $SU(n)\times (\Pbasic)_T$ under the relation $(g, v_1\wedge \cdots \wedge v_k) \sim (gt^{-1}, tv_1 \wedge \cdots \wedge tv_k)$ for $t\in T$. 
Having defined this bundle gerbe, we can now present one of the key results from this section.
\begin{proposition}[\cite{53UNITARY}]\label{iso1} 
	There is a bundle gerbe isomorphism $$ \left(  \PbasicT \times_T SU(n), Y_T\times \su, T\times \su \right)\to \pullbackbasicbg.$$  
\end{proposition} 
\begin{proof} It is clear by Equation \eqref{eq:test} that $Y_T\times \su \cong p^{-1}(Y)$, and that this identification is a smooth isomorphism of surjective submersions over $T\times \su$. It follows that $Y_T^{[2]} \times \su \cong p^{-1}(Y)^{[2]}$ and this diffeomorphism covers $Y_T\times \su \xrightarrow{\sim} p^{-1}(Y).$ 
It remains to define a line bundle isomorphism (that respects the bundle gerbe multiplication) between the line bundles present in these bundle gerbes, depicted in Figure \ref{fig:pullbackpf}.  \begin{figure}[h!] 
	\begin{center} 
		\begin{tikzcd}
			\PbasicT \times_T SU(n) \arrow[r, "f"]  \arrow[d]	& 	(\hat{p}^{[2]})^{-1}(\Pbasic)  \arrow[d]	  \\		
				Y_T^{[2]}\times \su \arrow[r, "\sim"]&	{p}^{-1}(Y)^{[2]}
		\end{tikzcd} 
		\caption{Isomorphism of line bundles }
		\label{fig:pullbackpf} \end{center} \end{figure}
We do so by considering the connected components of $Y_T^{[2]}$. Let $Y_{T, +}^{[2]}, Y_{T, 0}^{[2]}$ and $Y_{T, -}^{[2]}$ denote the restriction of $Y_{+}^{[2]}, Y_{0}^{[2]}$ and $Y_{-}^{[2]}$ to $Y_T^{[2]}$ respectively.
  Let $(z_1, z_2, t) \in Y^{[2]}_{T, +}$ and $ v_1\wedge \cdots \wedge v_k\in (\PbasicT)_{(z_1, z_2, t)}$. Then each $v_i$ is an eigenvector of $t$ with eigenvalue $\lambda_i$, say. Recall from earlier that multiplication by $g$ gives a map $L_{(z_1, z_2, t)}\to L_{(z_1, z_2, gtg^{-1})}$. This in turn induces a (linear) map 
\begin{align*}
(\PbasicT)_{(z_1, z_2, g)} &\to (\PbasicT)_{(z_1, z_2, gtg^{-1})}\\
v_1\wedge \cdots \wedge v_k &\mapsto gv_1\wedge \cdots \wedge gv_k.
\end{align*} 
Finally, define $f:\PbasicT\times_T SU(n) \to (\hat{p}^{[2]})^{-1}(\Pbasic)$ over fibres $(gT, z_1, z_2, t) \in Y_{T, +}^{[2]}\times \su$ by  $$[v_1\wedge \cdots \wedge v_k, g]  \mapsto (gT, t, z_1, z_2, gv_1 \wedge \cdots \wedge gv_k).$$
This map is well-defined by definition of the $T$-action on $\PbasicT\times SU(n)$. It is also clearly a linear isomorphism on fibres covering $Y_{T, +}^{[2]}\times \su  \xrightarrow{\sim} p^{-1}(Y)$. By duality, we can extend $f$ to $Y_{T, -}^{[2]}\times \su$ so that it remains a linear isomorphism on fibres over $Y_{T, -}^{[2]}\times \su$ and covers $Y_{T, -}^{[2]}\times \su \xrightarrow{\sim} p^{-1}(Y)^{[2]}$. Trivially, we can extend $f$ to $Y_{T, 0}^{[2]}\times \su$. It can be verified that $f$ commutes with the bundle gerbe multiplication, so is the desired line bundle isomorphism. \end{proof} 
We summarise our finding in Figure \ref{fig:pullbacktriple}. Since they are isomorphic, the two bundle gerbes from the previous proposition are stably isomorphic (Remark \ref{remark isoimplies stable iso}). 
\begin{figure}[h!] 
	\begin{center} 
		\begin{tikzcd}[row sep = 2em, column sep=3em]
		 \PbasicT \times_T SU(n) \arrow[r, "\sim"]  \arrow[d]	& 	(\hat{p}^{[2]})^{-1}(\Pbasic) \arrow[r]  \arrow[d]		  &\Pbasic \ \  \arrow[d, shift right = .7ex]   \\
		Y_T^{[2]}\times \su \arrow[r, "\sim"] \arrow[d, shift right=1.2ex] \arrow[d,shift left=.1ex]&	{p}^{-1}(Y)^{[2]} \arrow[r, "\hat{p}^{[2]}"] \arrow[d, shift right=1.2ex] \arrow[d,shift left=.1ex]& Y^{[2]}  \arrow[d, shift right=1.2ex] \arrow[d,shift left=.1ex] \\
			Y_T \times \su \arrow[r, "\sim"]  \arrow[d]&	p^{-1}(Y)  \arrow[r, "\hat{p}"] \arrow[d] &  Y \  \  \arrow[d, shift right = .7ex] \\ 
			T\times \su \arrow[r, equal] &	T\times \su \arrow[r, " \ \ \ p"] & SU(n) \ \ 
			
		\end{tikzcd} 
		\caption{Isomorphism of $\pullbackbasicbg$ }
		\label{fig:pullbacktriple} \end{center} \end{figure}
\begin{remark}
It can be easily shown that the isomorphism in Proposition \ref{iso1} is in fact $SU(n)$-equivariant by considering the $SU(n)$-action on $\left(\PbasicT \times_T SU(n), Y_T\times \su\right)$ from Remark \ref{remark equivariance of other bundle gerbe} and the pullback of the $SU(n)$-actions on $\basicbg$ from Proposition \ref{proposition basic bg is equivariant}.
\end{remark}





%dentify the spaces $p^{-1}(Y), p^{-1}(Y)^{[2]}$ and $\LL\hat{p}^{[2]}\RR^{-1}(L)$ with those in Equations  \eqref{eq:test}, \eqref{eq:test2}, and \eqref{eq:test3} respectively. %Note that the surjective submersions in the given bundle gerbes are defined as \begin{align*}
%\pi_1: \su\times Y_T\to \su \times T , \ \ \ \ (gT, (z, t)) \mapsto (gT, t)
%\end{align*}
%and 
%\begin{align*}
%\pi_2: p^{-1}(Y)\to \su \times T, \ \ \ \ (gT, t, z)\mapsto (gT, t). 
%\end{align*}
%Define a map \begin{align*} 
%p_Y: \Su \times Y_T \to p^{-1}(Y) \\
%(gT, z, t) \mapsto (gT, t, z). 
%\end{align*} We claim $p_Y$ is a smooth isomorphism of surjective submersions. Certainly $p_Y$ is smooth and makes the diagram 	 \[\begin{tikzcd}[column sep=small]
%\Su \times Y_T \arrow[dr, "\pi_1", swap] \arrow{rr}{p_Y} & & p^{-1}(Y) \arrow[dl, "
%\pi_2"] \\
%& \Su\times T &
%\end{tikzcd}\] commute, where $\pi_1$ maps an element $(gT, (z, t))\in \su \times Y_T$ to $(gT, t)\in \su \times T$ and $\pi_2$ maps an element $(gT, t, z) \in p^{-1}(Y)$ to $(gT, t)\in \su\times T$. Also, $p_Y$ is a smooth morphism of surjective submersions. It is easy to check that the map $$p^{-1}(Y)\to \Su\times Y_T, \ \ \ (gT, t, (z, s)) \mapsto (gT, (z, t)) $$
%is a smooth morphism surjective submersions and is an inverse to $p_Y$, therefore $p_Y$ is a smooth isomorphism of surjective submersions, as required. \\ \text{}\\


%\textit{Proof.} By the universal property of the pull back of bundle gerbes combined with the previous result we obtain a bundle gerbe morphism of the form $\left(\alpha, \beta, id\right)$ between the desired bundle gerbes. By {\color{blue}{insert propn numnber}} this implies the above bundle gerbes are stably isomorphic.  
Define, for each $i=1, ..., n$, the map $p_i : T\to S^1$ which maps $t\in T$ to its $i$-th diagonal element. 
\begin{definition}\label{defnepsilon}
	Define $\varepsilon_i: Y_T^{[2]}\to \Z$ by $$\varepsilon_i(z_1, z_2, t) = \begin{cases}
	1 & \text{if } z_1 > p_i(t) > z_2 \\
	-1 & \text{if } z_2 > p_i(t) > z_1 \\ 
	0 & \text{otherwise}.
	\end{cases} $$
\end{definition}
\begin{center}
	\begin{tikzpicture}\centering 
	\draw (0, 0) circle (1.5 cm);
	\draw[fill = black] (1, 1.118) circle (2pt);
	\draw[fill = black] (0, -1.5) circle (2pt);
	\draw[fill = white, draw = black] (1.5, 0) circle (2pt);
	\node[] at (1.28, 1.3) {$z_1$};
	\node[] at (0, -1.85) {$z_2$};
	\draw[fill = black] (-1, 1.118) circle (2pt);
	%\draw[fill = black] (-1.414, -.5) circle (2pt);
	\node[] at (-1.2, 1.35) {$t$};
	%\node[] at (-1.7, -.6)  {$t_2$};
	\node[] at (0, -2.7) {$\varepsilon(z_1, z_2, t) = -1$};
	
	
	\draw (6, 0) circle (1.5 cm);
	\draw[fill = black] (7, 1.118) circle (2pt);
	\draw[fill = black] (4.585, -.5) circle (2pt);
	\draw[fill = black] (5, 1.118) circle (2pt);
	\draw[fill = white, draw = black] (7.5, 0) circle (2pt);
	\node[] at (7.28, 1.3) {$z_2$};
	\node[] at (4.3, -.6) {$z_1$};
	\node[] at (4.8, 1.35) {$t$};
	\node[] at (1, 1) {};
	\node[] at (6, -2.7) {$\varepsilon(z_1, z_2, t) = 1$};
	
	\draw (12, 0) circle (1.5 cm);
	\draw[fill = black] (12, -1.5) circle (2pt);
	\draw[fill = black] (12, 1.5) circle (2pt);
	\draw[fill = black] (12.9, 1.2) circle (2pt);
	\draw[fill = white, draw = black] (13.5, 0) circle (2pt);
	\node[] at (12, 1.8) {$z_2$};
	\node[] at (12, -1.8) {$t$};
	\node[] at (13.17, 1.37)  {$z_1$};
	\node[] at (1, 1) {};
	\node[] at (12, -2.7) {$\varepsilon(z_1, z_2, t) = 0$};
	\end{tikzpicture} \end{center}

We next aim to better understand $L_T \to Y_T^{[2]}$ which will allow us to ultimately find a simple description for the pull back of the basic bundle gerbe via the Weyl map. Let $(z_1, z_2, t) \in Y_{T, +}^{[2]}$. Then the $p_i(t)$-eigenspace of $t$ is $$E_{(t, p_i(t))} = \text{span}(e_i) \cong \C$$ where $e_i$ is the $i$-th standard basis vector of $\C^n$. Of course $E_{(t, \lambda)} = \{0\}$ if $\lambda \neq p_i(t)$ for each $i=1, ..., n$. %Therefore the $\lambda$-eigenspace of $t$ is $$E_{(t, \lambda)} = \begin{cases}
%\C& \text{if } \lambda = t_i \text{ for some } i \\
%\{0\} & \text{otherwise}.
%\end{cases} $$  {\textcolor{red}{check}} 
Let $p_{k_1}(t), ..., p_{k_m}(t)$ be all of the eigenvalues of $t$ between $z_1 > z_2$ for $m, k_1, ..., k_m \in \{1, ..., n\}$. Then 
$$
(\PbasicT)_{(z_1, z_2, t)} = \text{det}(L_{(z_1, z_2, t)}) = \Motimes_{z_1 >\lambda > z_2} \text{det} \left(E_{(t, \lambda)}\right)=E_{(t, p_{k_1}(t))}\otimes \cdots \otimes E_{\left(t,p_{k_m}(t)\right)}.
$$ 
Now, each eigenspace $E_{(t, p_k(t))} \cong \C$ is equipped with a $T$-action $s\cdot v := p_k(s) v$, multiplication by the $k$-th diagonal element of $s$. To ease notation, for each $k=1, ..., n$ define $\C_{p_k}$ to be $\C$ equipped with the $T$-action $s\cdot v := p_k(s)v$. So $E_{(t, t_ik} \cong \C_{p_k}$ as $T$-spaces for each $k$. Therefore $$ \left(\PbasicT\right)_{(z_1, z_2, t)} \cong \C_{p_{i_1}} \otimes \cdots \otimes \C_{p_{i_k}}.$$ 
%Recall that $T$ acts on an element $v_1\wedge \cdots \wedge v_n$ by $t\cdot v_1\wedge \cdots \wedge v_n := tv_1\wedge \cdots \wedge tv_n = t_1v_1 \wedge \cdots \wedge t_n v_n$.  
If we instead assume $(z_1, z_2, t) \in Y_{T, -}^{[2]}$ with $t_{i_1}, ..., t_{i_k}$ all of the eigenvalues of $t$ between $z_2>z_1$, by almost identical arguments we find $$ \left(L_T\right)_{(z_1, z_2, t)} \cong \C_{p_{i_1}}^* \otimes \cdots \otimes \C_{p_{i_k}}^*. $$ Therefore, for any $(z_1, z_2, t)\in Y_T^{[2]}$, we have $$ \left(L_T\right)_{(z_1, z_2, t)} \cong \C_{p_{1}}^{\varepsilon_1(z_1, z_2, t)} \otimes \cdots \otimes \C_{p_{n}}^{\varepsilon_n(z_1, z_2, t)} $$ using the maps $\varepsilon_i$ as in Definition \ref{defnepsilon}. The maps $\varepsilon_i$ effectively `pick out' the diagonal elements $t_i$ of $t$ between $z_1$ and $z_2$, and assign to them $\C_{p_i}$ or $\C_{p_i}^*$ depending on whether $z_1>z_2$ or $z_2>z_1$. So we may express the trivial line bundle $L_T\to Y_T^{[2]}$ as $$L_T \cong \C_{p_1}^{\varepsilon_1}\otimes \cdots \otimes \C_{p_n}^{\varepsilon_n}\times Y_T^{[2]}.$$ Let $U\subseteq Y_T^{[2]}$ be a connected component. By continuity of the integer-valued maps $\varepsilon_i$, there are $k_1, ..., k_n\in \{-1, 0, 1\}$ for which $\varepsilon_i|_U = k_i$ for each $i=1, ..., n$. Define
\begin{align*} \C_{{p_i},k} := \begin{cases} \C_{p_i}& \text{if } k = 1\\
\C&\text{if } k=0\\
\C_{p_i}^* & \text{if } k = -1.
\end{cases} \end{align*} 
So $$\left(L_T\right)|_U\cong \C_{{p_1},{k_1}}\otimes\cdots \otimes  \C_{{p_n},{k_n}}\times U.$$
%Let $U\subseteq Y_T^{[2]}$ be a connected component. Since $\varepsilon_i$ is a continuous and integer valued, there exists $n_i \in \Z$ such that $\varepsilon_i|_{U} = n_i$ for $i= 1, ..., n$.  
Recall the line bundles $J_i  := \C\times SU(n)/\sim_{p_i}$ over $\frac{SU(n)}{T}$ defined for each $i=1, ..., n$ by the relation $(z, s) \sim_{p_i} (p_i(t^{-1})z, st)$ for 
$(z,s) \in  U(1)\times SU(n)$ and $t\in T$. We can similarly define the $SU(n)$-homogeneous line bundle $J_{i,k} := \C_{{p_i},k} \times SU(n)/\sim_{p_i}$ over $SU(n)/T$. 
\begin{proposition}\label{Jiso}
	Let $(L, Y, SU(n))$ be the basic bundle gerbe. The pull back of $L\to Y^{[2]}$ by the Weyl map $p$ is isomorphic to $J_{1}^{\varepsilon_1}\otimes \cdots \otimes J_{n}^{\varepsilon_n} \to \su \times Y_T$. 
\end{proposition}
\begin{proof} First, note that $$\frac{\C_{p_1,k_1} \otimes \cdots \otimes \C_{p_n,k_n} \times SU(n) }{T} \cong J_{1,k_1} \otimes \cdots \otimes J_{n,k_n} $$ as $SU(n)$-homogeneous line bundles over $SU(n)/T$. This follows by Theorem \ref{thrmbundles} because the associated linear representations of $T$ for each of these line bundles is the same. Let $U\subseteq Y_T^{[2]}$ be a connected component. Then it can be verified that the map $$\frac{(\C_{p_1,k_1} \otimes \cdots \otimes \C_{p_n,k_n}\times U) \times SU(n) }{T} \to U \times \frac{\C_{p_1,k_1} \otimes \cdots \otimes \C_{p_n,k_n} \times SU(n) }{T} $$ given by $[(v, u), g] \mapsto (u, [v, g])$ is well defined and gives an isomorphism between these line bundles over $U \times SU(n)/T$. So by these results and Proposition \ref{iso1} we have the following isomorphisms of line bundles: \begin{align*}
p^{-1}(L)|_U &\cong \frac{L_T|_U\times SU(n)}{T}\\
&\cong \frac{(\C_{p_1,k_1} \otimes \cdots \otimes \C_{p_n,k_n}\times U) \times SU(n) }{T} \\
&\cong  U \times \frac{\C_{p_1,k_1} \otimes \cdots \otimes \C_{p_n,k_n} \times SU(n) }{T} \\
&\cong U\times  (J_{1,k_1} \otimes \cdots \otimes J_{n,k_n}) \\
&\cong (J_{1}^{\varepsilon_1} \otimes \cdots \otimes J_{n}^{\varepsilon_n})\big\rvert_{U\times SU(n)/T}. 
\end{align*} {\textcolor{red}{is my notation for $J^\epsilon$ consistent with my defn of raising a line bundle to power of a function? Think about this. }}As this is true for each connected component $U\subseteq Y^{[2]}_T$, we obtain the result. \end{proof} 
	\section{Connective structure on the basic bundle gerbe}
	\indent \indent A canonical bundle gerbe connection can be constructed on the basic bundle gerbe $(L, Y, SU(n))$ as follows \cite{53UNITARY}. We do so by first considering the connection $\nabla$ on $E|_{Y_+^{[2]}}\subset \C^n\times Y_+^{[2]}$ induced by the trivial connection, $P(d)$, for $P:\C^n\to E$ orthogonal projection. This gives rise to a connection det$(\nabla)|_{Y_+^{[2]}}$ on $L|_{Y_+^{[2]}}$. The dual connection and trivial connection give us connections on $L|_{Y_-^{[2]}}$ and $L|_{Y_0^{[2]}}$ respectively, thereby defining a connection det$(\nabla)$ on all of $L$. We claim $\text{det}(\nabla)$ is a bundle gerbe connection on $(L, Y, SU(n))$. Consider a connected component of $U\subset Y^{[3]}_{(1,1)}$ containing some $(z_1, z_2, z_3, g)$ with $z_1>z_2>z_3$. {\textcolor{red}{define this.}} Recall Equation \ref{eqn3} that over $U$ $$E_{(z_1, z_2, g)} \oplus E_{(z_2, z_3, g)} = E_{(z_1, z_3, g)}.$$ Therefore over $U$ we have $$\pi_2^{-1}(E) = \pi_3^{-1}(E)\oplus \pi_1^{-1}(E).$$ Since the latter is an orthogonal splitting and $\nabla$ is defined by orthogonal projection we have $$\pi_2^{-1}(\nabla) = \pi_3^{-1}(\nabla) \oplus \pi_1^{-1}(\nabla). $$ Therefore the wedge product gives us the isomorphism $$\pi_2^{-1}(\text{det}(\nabla)) = \pi_3^{-1}(\text{det}(\nabla)) \otimes \pi_1^{-1}(\text{det}(\nabla)). $$ This implies $\text{det}(\nabla)$ respects the bundle gerbe multiplication over $U$. By similar arguments, $\text{det}(\nabla)$ respects the bundle gerbe multiplication on the other connected components of $Y^{[3]}$,  hence is a bundle gerbe connection on $L$. Finally, by Example \ref{linebundlecurvature}, $F_\nabla s= PdPdPs$ for $s\in \Gamma(Y^{[2]}, E)$ and $$F_{\text{det}(\nabla)} s = \text{tr}(PdPdP)s. $$ 
	
	% By Example \ref{linebundlecurvature}, the trivial connection on $\C^n\times Y^{[2]}_+$ induces a connection $\nabla$ on $E$ with curvature $$F_\nabla s = PdPdPs $$ for $P:\C^n\times Y^{[2]}_+ \to E$ orthogonal projection and $s\in \Gamma(M, E)$. 
	
	%Note that $L|_{Y_+^{[2]}} \to Y_+^{[2]}$ is a subbundle of the trivial bundle of rank $n$ over $Y_+^{[2]}$. Therefore Example \ref{linebundleconnection} applies and we obtain a line bundle connection $\text{det}(\nabla)$ on $L_+^{[2]}$. The dual connection and trivial connection give us connections on $L|_{Y_-^{[2]}}$ and $L|_{Y_0^{[2]}}$ respectively, thereby defining a connection det$(\nabla)$ on all of $L$. We claim $\text{det}(\nabla)$ is a bundle gerbe connection on $(L, Y, SU(n))$.  
	%{\textcolor{red}{the following argument is in the paper, ask if this can be adapted using the fact that $\pi_2^*(L) = \pi_3^*(L)\otimes \pi_1^*(L).$}}
%	Let $(z_1, z_2, z_3, g) \in Y^{[3]}_{(1, 1)}$ {\textcolor{red}{define this space earlier}} with $z_1>z_2>z_3$. Recall Similar arguments can be used to show $\nabla$ is a bundle gerbe connection on all of $E$. This implies $\text{det}(\nabla)$ is a bundle gerbe connection on $L$.
	%\text{}\\ \text{}\\ \text{}\\ 
	
	
	
%	The curvature two form of this connection is given by $F_\nabla = \text{tr}(PdPdP)$, where $P$ is orthogonal projection $Y^{[2]}\times \C^n \to L$ with respect to the Hermitian metric on $L$. We claim $\nabla$ is a bundle gerbe connection. 
	
%	By projecting the trivial connection on $Y_+^{[2]}\times \C^n$ onto $E$ we obtain a connection $\nabla s := P(ds)$ on $E$. This in turn defines a connection det$(\nabla)$ on $L|_{Y_+^{[2]}}$.  We claim this is a bundle gerbe connection.
	%{\textcolor{red}{is it obvious that the det of a bundle gerbe connection is again a BG connection}}
	%\indent Let $F_\nabla$ denote the curvature two form of the connection $\nabla$ on $E$. It is a standard fact that the curvature two form on $L$, denoted by $F_{\text{det}(\nabla)}$ is equal to the trace of $F_\nabla$. We compute $F_\nabla$ explicitly in terms of $P$ as follows. 
	%Let $s_\alpha: Y_+^{[2]}\to E$ be a local nowhere vanishing section and define a one form $A_\alpha$ on $U_\alpha$ implicitly by $\nabla s_\alpha = A_\alpha s_\alpha$. So the curvature two form $F_\nabla$ is locally equal to $dA_\alpha$. 
	
	%Therefore $F_\nabla = PdPdP$ and \begin{align*}F_{\text{det}(\nabla)} = \text{tr}(PdPdP).\end{align*}
	%The proceeding Theorem describe the curving and $3$-curvature of the basic bundle gerbe. {\textcolor{red}{how to cite a theorem}} 
	\begin{theorem}\label{theorem basic bundle gerbe data} \cite{53UNITARY}
		Let $f$ be a two-form on $Y$ defined by the contour integral 
		$$f(z, g) = \frac{1}{8 \pi^2} \int_{C_{(z,g)}} \text{log}_z\zeta \text{tr}\left((\zeta-g)^{-1}dg(\zeta-g)^{-2}dg\right)d\zeta. $$ Then \begin{enumerate}[(1),font=\upshape]
			\item the two form $f$ satisfies $\delta(f) = F_{\text{det}(\nabla)}$, so $f$ is a curving for the bundle gerbe connection det$(\nabla)$;
			\item the three curvature of the bundle gerbe connection det$(\nabla)$ is given by $$\omega = -\frac{i}{12\pi}\text{tr}(g^{-1}dg)^3 $$ for $g\in SU(n)$ the standard coordinate chart; 
			\item the Dixmier-Douady class of the basic bundle gerbe is $$\nu= -\frac{1}{24\pi^2}\text{tr}(g^{-1}dg)^3. $$ 
		\end{enumerate}
	\end{theorem}
	The form in $(3)$ is the canonical closed three-form on $SU(n)$, called the \textit{basic three form}.  \\ 
\indent \indent	The three curvature of the pull back of the basic bundle gerbe by the Weyl map $p$ is equal to $p^*(\omega) = p^*(2\pi i \nu)$. To relate this to the three curvature of the cup product bundle gerbe, we write $p^*(2\pi i \nu)$ in terms of orthogonal projections. To do so, we must first understand the Weyl map in terms of projections.\\ 
	Using this description of the Weyl map, we obtain the following proposition. \begin{proposition} [\cite{53UNITARY}] \label{curvature} The three curvature of the pull back of the basic bundle gerbe by the Weyl map, $p^*(2\pi i \nu)$, is equal to  \begin{align*} \frac{i}{4\pi} \sum_{i\neq k} \left(p_i^{-1} dp_i - dp_k p_k^{-1} -p_k^{-1}dp_i + p_k^{-1}dp_k p_k^{-1}p_i\right) \text{tr}(P_idP_kdP_k) - \frac{i}{4\pi}  \sum_{i\neq k} p_ip_k^{-1} \text{tr}(dP_idP_kdP_k). \end{align*} {\textcolor{red}{not sure how to explain what projections are in this general setting}} \end{proposition} 
	
	
	\chapter{Cup product bundle gerbe}
	In the proceeding example we construct the \textit{cup product} bundle gerbe, which will be central to our research. The definition of the cup product bundle gerbe is motivated by the cup product map of \v{C}ech cocycles. Given sheaves of abelian groups $F$ and $G$, the cup product
	$$\cup: C^p(\mathcal{U}, F)\otimes C^{q}(\mathcal{U}, G) \to C^{p+q}(\mathcal{U}, F\otimes G)$$ is defined by mapping  $(\underline{\alpha}, \underline{\beta})\mapsto \underline{\alpha}\cup \underline{\beta}$ where $$(\underline{\alpha}\cup \underline{\beta})_{i_0, ..., i_{p+q}} := \alpha_{i_0, ..., i_p}\otimes \beta_{i_q, ..., i_{p+q}}. $$ In particular, taking $F = \Z(1)_D$, $Q = \Z(2)_D$, $p=1$ and $q=2$, the cup product induces a map of \v{C}ech hypercohomology groups, and hence of sheaf hypercohomology groups, \begin{align}\label{eqn cup product} \cup: H^1(M, \Z(1)_D)\otimes H^{2}(M, \Z(2)_D) \to H^{3}(M, \Z(3)_D).\end{align} 
	Recall that smooth maps $f:M\to U(1)$, line bundles with connection, and bundle gerbes with connective structure are classified by $H^1(M, \Z(1)_D)$, $H^{2}(M, \Z(2)_D)$, and $H^3(M, \Z(3)_D)$ respectively (Remark \ref{remark deligne cohomology of line bundles and functions}). Therefore by Equation \ref{eqn cup product} we expect the cup product to define a bundle gerbe $(f\cup L, Y, M)$ given a map $f: M\to U(1)$ and a line bundle $L\to M$ with connection. Of course, the Deligne class of $(f\cup L, Y, M)$ will then equal the cup product of Deligne classes of $f$ and $L\to Y$.
	
	
	This construction describes how a bundle gerbe can be formed given a smooth map $M\to S^1$ and a line bundle over $M$. The set up is as follows. Let $M$ be a smooth manifold, $\pi: P\to M$ be a line bundle, and $f:M\to S^1$ be a smooth map. Let $\R\to S^1$ be the principal $\Z$-bundle with projection $x\mapsto [x]$ the quotient map by $\Z$. The given information is depicted below.% As we shall see, the map $f:M\to S^1$ allows us to construct a bundle gerbe over $M$ from a line bundle over $M$. 
	
	\begin{center} 
		\begin{tikzcd}
			P  \arrow[swap]{d}{\pi}       
			&\R \arrow{d}{[\cdot]} \\
			M  \arrow[swap]{r}{f}
			&S^1
		\end{tikzcd} 
		\text{}\\ \text{}\\ { \color{red}{Label this diagram }} 
	\end{center}
	By pulling back $\R \to S^1$ along $f$, we obtain a $\Z$-bundle $f^{-1}(\R)$ over $M$. The space $f^{-1}(\R)$ consists of pairs $(m, t) \in M\times \R$ with $f(m) = [t]$. By Example \ref{fibreproductexample} the second fibre product of $f^{-1}(\R)$ consists of triples $(m, t_1, t_2)\in M\times \R\times \R$ with $f(m) = [t_1]=[t_2]$. Let $d: f^{-1}(\R)^{[2]}\to \Z$ be the difference map $d(m, t_1, t_2) = t_1-t_2$. Let $\pi_M: f^{-1}(\R)^{[2]} \to M$ be projection. Define a line bundle $P\cup f\to f^{-1}(\R)^{[2]}$ by $$P\cup f := \pi_M^{-1}\left(P\right)^d$$ using the notation from Example \ref{powerlinebundles}. To be completely explicit, for $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$, $$(P\cup f)_{(m, t_1, t_2)} = (P_m)^{d(m,t_1, t_2)}.$$ We claim the triple $(P\cup f, f^{-1}(\R), M)$ is a bundle gerbe. The space $P\cup f$ is indeed equipped with a natural bundle gerbe multiplication. Let $(m, t_1, t_2, t_3) \in Y^{[3]}$.  Then \begin{align*}
	\pi_1^{-1}(P\cup f)\otimes \pi_3^{-1}(P\cup f)_{(m, t_1, t_2, t_3)} 
	&= (P_m)^{t_2-t_3}\otimes (P_m)^{t_1-t_2}\\
	&= (P_m)^{t_1-t_3}\\
	&= \pi_2^{-1}(P\cup f)_{(m, t_1, t_2, t_3)}. 
	\end{align*} This map is certainly a smooth isomorphism of line bundles. Associativity of the bundle gerbe multiplication  follows from associativity of the tensor product of line bundles. 
	\begin{definition}  Given a smooth manifold $M$, a smooth map $f: M\to S^1$, and a line bundle $P\to M$, the triple $(P \cup f, f^{-1}(\R), M)$ constructed above is a bundle gerbe, called the \textit{cup product bundle gerbe}. \end{definition} {\color{red}{give motivation for name by talking about DD class}} 
	\begin{center} 
		\begin{align*}
		\begin{array}{ccc}
		P \cup f      &              \\
		\downarrow &               \\
		f^{-1}(\R)^{[2]}   & \stackrel{}{\dra} f^{-1}(\R) \\
		&                   \downarrow  \\
		&                    M      \\
		\end{array}
		\end{align*}
		{\color{red}{label diagram}} 
	\end{center}
	\begin{remark}\label{isoZ}
		Note that $f^{-1}(\R)^{[2]} \cong f^{-1}(\R)\times \Z$. This follows since $(m, t_1, t_2) \in f^{-1}(\R)^{[2]}$ if $f(m) = [t_1] =[t_2]\in S^1$. The latter equality holds if and only if $t_1-t_2\in \Z$. So by identifying an element $(m, t_1, t_2)\in f^{-1}(\R)^{[2]}$ with $(m, t_1, t_1-t_2) \in  f^{-1}(\R)\times \Z$ we obtain the desired diffeomorphism. 
	\end{remark}
	\begin{example}\label{ex 1}
		In this example we look at a specific instance of the cup product bundle gerbe. We shall first define a line bundle over $T\times \su$, and will obtain from this a bundle gerbe over $T\times \su$ using the cup product construction. Let $T$ be the maximal torus of $SU(n)$ defined by $$T := \{\text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}) : \ x_1 + \cdots + x_n = 0\}\cong \left(S^1\right)^{n-1}. $$ For $i = 1, ..., n$, define the group homomorphism $$ {p}_i: T\to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n})  \mapsto e^{2\pi i x_i}.$$ For each $i=1, ..., n$, define a line bundle $\pi: {J}_i \to \frac{SU(n)}{T}$ by $${J}_i = SU(n)\times \C/\sim_{{p}_i}, $$ where $(s, z)\sim_{{p}_i} (st, {p}_i(t^{-1})z)$ for all 
		$(s, z) \in SU(n)\times U(1)$ and $t\in T$.  Denote equivalence classes in $J_i$ by $[\cdot, \cdot]_{p_i}$. It follows  that the projection $\pi: [(s, z)] \mapsto sT$ is a well-defined surjective submersion. We abuse notation and denote the pullback of $J_i$ along the projection $T\times \su \to \su$ by $J_i\to T\times \su$ throughout this work. Consider the map $$p_i: T\times\su \to S^1, \ \text{diag}(e^{2\pi i x_1}, ..., e^{2\pi i x_n}, gT)\mapsto e^{2\pi i x_i}$$ defined for $i=1, ..., n$. 
		
		
		%	Consider the projection $$\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su\to \su$$ and define a line bundle ${J}_i \to T\times \su$ by $$J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}{J}_i'.$$
		%	%Using the constant identity-valued map $\textbf{1}_n: J_i\to T$, we can consider $J_i$ as a line bundle over $T\times \su$ with projection $1\times \pi$. 
		The elements that will be used to construct the cup product bundle gerbe are depicted below. 
		
		\begin{figure}[h!] 
			\begin{center} 
				\begin{tikzcd}
					J_i  \arrow[swap]{d}{}      
					&\R   \arrow{d}{[\cdot]}  \\
					T\times \frac{SU(n)}{T}\arrow[swap]{r}{p_i}
					&S^1
				\end{tikzcd}  \caption{Cup product bundle gerbe set up}
				\label{fig:pb1} \end{center}\end{figure} 
		%$J_{i,  {\smath{ \dfrac{SU(n)}{T} } }}, J_{i, T\times {\smath{ \dfrac{SU(n)}{T} } }}$ {\textcolor{red}{FINISH NEATENING UP NOTATION}}	Lastly, by pulling back $\R\to S^1$ by $p_i$ as before 
		Using the construction defined about, for each $i=1, ..., n$, we obtain a cup product bundle gerbe $$\left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$$ 
		%Consider the projection $$\pi_{T\times {\smath{ \dfrac{SU(n)}{T} } }}: p_i^{-1}(\R)^{[2]}\to T\times \su$$, 
		where, for any $(x_1, x_2,t,sT) \in p_i^{-1}(\R)^{[2]}$, we have $$(J_i \cup p_i)_{(x_1, x_2, t, sT)} = \left({J}_i \right)_{sT}^{x_1-x_2}.$$ %Since this fibre is independent of $t \in T$, we may sometimes abuse notation and write this fibre as $(J_i  \cup p_i)_{
		%	(x_1, x_2,sT)}$. 
		%$$(L_i\cup \varphi_i, \R^{n-1}\times  \tfrac{SU(n)}{T}, T\times  \tfrac{SU(n)}{T}). $$ {\color{red}{refer to figure}}   $$ \begin{array}{ccc}
		%L_i\cup \lambda_i         &          &        \\
		%\downarrow &         &         \\
		%\R^{n-1}\times \tfrac{SU(n)}{T}\times \Z  & \stackrel{}{\dra} &  \R^{n-1}\times \tfrac{SU(n)}{T} \\
		%&               &      \downarrow \\
		%&               &       T\times  \frac{SU(n)}{T}        \\
		%\end{array} $$
	\end{example} 
	In the following example, the product of these $n$ bundle gerbes is formed to construct a single bundle gerbe over $T\times \su$. The resulting bundle gerbe will be central to our research question. 
	\begin{remark}\label{isocup}
		%By remark \ref{isoZ}, we see that $p_i^{-1}(\R)^{[2]}\cong p_i^{-1}(\R)\times \Z$. We can also understand these spaces in terms of the original projection map $\widetilde{p}_i: T\to S^1$ as $$p_i^{-1}(\R)\cong \left(\widetilde{p}_i\right)^{-1}(\R)\times \su$$ and $$p_i^{-1}(\R)^{[2]} \cong \Z\times \left(\widetilde{p}_i\right)^{-1}(\R)\times \su.$$ 
		We can write the space $p_i^{-1}(\R)$ explicitly as $$p_i^{-1}(\R) = \left \{(t, gT, x)\in T\times \su \times \R \ \big \rvert \ t_i = [x]\right\}.$$ 
	\end{remark}
	\begin{proposition}\label{cupprodisequivariant} 
		The cup product bundle gerbes $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ defined above are $SU(n)$-equivariant for each $i=1, ..., n$. 
	\end{proposition}
	\textit{Proof}. Let us define the $SU(n)$ action on each of the spaces present in our bundle gerbe. On $T\times \su$, $SU(n)$ acts by $$g\cdot (t, hT) := (t, ghT). $$ On $p_i^{-1}(\R) = \left \{(x, t, hT) \in \R\times T\times \su \ | \ p_i(t) = [x]\right\}$, $SU(n)$ acts by $$g\cdot (x, t, hT) := (x, t, ghT), $$ and similarly for $p_i^{-1}(\R)^{[2]}$. Finally, for a standard element $\otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} \in (J_i\cup p_i)_{(x_1, x_2, hT)}$ the $SU(n)$-action is defined by $$g\cdot \otimes_{j=1}^{x_1-x_2} [h, v_j]_{p_i} := \otimes_{j=1}^{x_1-x_2} [gh, v_j]_{p_i}. $$ This can be extended by linearity to define an action on any element in $J_i\cup p_i$. With these actions, $SU(n)$-equivariance of the bundle gerbe follows easily. 
	
	\begin{example}\label{exxx}
		Consider the bundle gerbes $\left(J_i \cup p_i, p_i^{-1}(\R), T\times \frac{SU(n)}{T}\right)$ for $i= 1, ..., n$ as in Example \ref{ex 1}. To describe the product of these $n$ bundle gerbes, we must first understand the fibre product $$H = p_1^{-1}(\R) \times_{T\times \frac{SU(n)}{T} }\times \cdots \times_{T\times \frac{SU(n)}{T}} p_n^{-1}(\R).$$ Since the projection from $p_i^{-1}(\R) \subseteq \R\times \left(T\times \su\right)$ to $  T\times \su$ is simply projection onto the second factor, it is clear that $$H \cong \left\{(x_1, ..., x_n, t, gT)\in \R^n \times T\times \tfrac{SU(n)}{T} \ \big\rvert\ [x_i] = p_i(t)\ \forall \  i = 1, ..., n \right\}.$$ Since the product of the diagonal entries of $t$ equals one, the condition that $[x_i] = p_i(t)$ for each $i = 1, ..., n$ can equivalently be stated as $x_1 + \cdots + x_n \in \Z$. Using this condition, and noting that $t = \text{diag}([x_1], ..., [x_n])$,  we find $$H \cong \left\{(x_1, ..., x_n, gT) \in \R^n \times \tfrac{SU(n)}{T} \ \big\rvert \ \textstyle \sum_{i=1}^n x_i \in \Z\right\}.$$ Let $W := \{(x_1, ..., x_n) \in \R^n :  \textstyle \sum_{i=1}^n x_i \in \Z\}.$ Then $H \cong W
		\times \tfrac{SU(n)}{T}.$ We remark that under this identification, the surjective submersion $H\to T\times \su$ becomes $$(x_1, ..., x_n, gT) \mapsto (\text{diag}([x_1], ..., [x_n]), gT)$$ when written as a map $W\times \su \to T\times \su$.  Therefore the tensor product from $i=1, ..., n$ of the bundle gerbes from Example \ref{ex 1} can be written as \begin{align} \label{eqn} \left(\Motimes_{i=1}^n J_i \cup p_i, W\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right). \end{align} 
	\end{example} 
	In some instances, a bundle gerbe $(P, Y, M)$ can equivalently be viewed as a bundle gerbe $(P|_{X^{[2]}}, X, M)$ for some submanifold $X\subseteq Y$. This is in fact a result of the following theorem.
	
	\begin{theorem}[\cite{stableiso}] \label{stable iso} 
		Let $\pi_1: Y\to M$, $\pi_2: X\to M$ be surjective submersions, and $f: X\to Y$ a morphism of surjective submersions, ie. $\pi_1\circ f = \pi_2$. Then a bundle gerbe $(P, Y, M)$ is stably isomorphic to $(f^{-1}(P), X, M)$. 
	\end{theorem} 
	An important consequence of this theorem occurs when $f$ is the inclusion of a submanifold into a manifold. The resulting corollary makes precise when a bundle gerbe $(P, Y, M)$ can equivalently be viewed as the bundle gerbe $(P|_{X^{[2]}}, X, M)$ for a submanifold $X\subset Y$. 
	
	
	\begin{corollary}\label{ex 2} 
		Consider a bundle gerbe $(P, Y, M)$ and a submanifold $X\subset Y$ such that $\pi|_X:X\to M$ is a surjective submersion. Let $\iota: X\to Y$ be inclusion. Then $\pi\circ \iota = \pi|_X$, therefore by Theorem \ref{stable iso} $(P, Y, M)$ is stably isomorphic to $(P|_{X^{[2]}}, X, M)$. 
	\end{corollary}
	This Corollary is most useful when the submanifold $X$ of $Y$ simplifies calculations on the bundle gerbe.  This is in fact the case for the bundle gerbe (\ref{eqn}), where the space $W \times \su$ can be replaced by the (simpler) space $\R^{n-1}\times \su$. We return to Example \ref{exxx} to make this precise. \\
	
	\noindent\textbf{Example 1.32. (Continued)} Let us justify why the space $W\times \su$ present in the bundle gerbe (\ref{eqn}) can be replaced with the space $\R^{n-1}\times \su$. First, note that $\R^{n-1}$ can be viewed as a submanifold of $W$ under the identification $$\R^{n-1} \cong \left\{(x_1, ..., x_n) \in \R^n \ \big\rvert \  \textstyle\sum_{i=1}^n x_i = 0\right\} \subseteq W.$$ Recall that the projection $W\times \su \to T\times \su$ is defined by $$ (x_1, ..., x_{n}, gT) \mapsto \left(\text{diag}\left([x_1], ...,  [x_n]\right), gT\right).$$ This map remains a surjective submersion when restricted to $\R^{n-1}\times \su$ because $T\cong (S^1)^{n-1}$. Therefore by Corollary \ref{ex 2}, the bundle gerbe (\ref{eqn}) is stably isomorphic to  $$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right) .$$
	Let us understand what this bundle gerbe looks like fibrewise. Since the projection map $\R^{n-1}\times \su \to T\times \su$ is the identity on the $\su$ factor, we have $$\left(\R^{n-1}\times \su\right)^{[2]} \cong \left(\R^{n-1}\right)^{[2]}\times \su$$ where the fibre product $\left(\R^{n-1}\right)^{[2]}$ is taken with respect to the projection $\R^{n-1}\to \left(S^1\right)^{n-1}$ given by $(x_1, ..., x_{n-1})\mapsto ([x_1], ..., [x_{n-1}])$. Let $(x, y, gT)\in \left(\R^{n-1}\right)^{[2]}\times \su$. Write $x$ and $y$ as $n$-tuples $(x_1, ..., x_n)$ and $(y_1, ..., y_n)$ respectively, whose coordinates sum to zero. Then  \begin{align}
	\left(\Motimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (J_1\cup p_1)_{(x_1, y_1, gT)} \otimes \cdots \otimes (J_n\cup p_n)_{(x_n, y_n, gT)}  \nonumber  \\
	&= (J_1)_{gT}^{d(x_1, y_1)}\otimes \cdots \otimes (J_n)_{gT}^{d(x_n, y_n)}.\label{Jifibres}
	\end{align}
	% Define for each $i=1, ..., n$ the map $p_i: \R^{n-1}\to \R$ defined by $p_i(x^1, ..., x^n)= x^i$ where again we identify $\R^{n-1}$ with the the subset of $\R^n$ whose coordinates sum to zero. Then \begin{align*}
	%\left(\bigotimes_{i=1}^n J_i \cup p_i\right)_{(x, y, gT)} &= (L_1)_{gT}
	% \end{align*}
	
	The following proposition follows immediately from Propositions \ref{equivariantbundlegerbeproduct} and \ref{cupprodisequivariant}.
	\begin{proposition}
		The bundle gerbe $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ defined above is $SU(n)$-equivariant. 
	\end{proposition}
	\subsection{Geometry of the flag manifold}
	
	\indent \indent Let $F_n$ be the manifold whose points are sets $\{W_1, ..., W_n\}$ of mutually orthogonal one-dimensional subspaces of $\C^n$ ($F_n$ is the \textit{flag manifold} of $\C^n$). Let $e_1, ..., e_n$ be the standard basis vectors of $\C^n$ and define the \textit{standard element} $e$ of $F_n$ by $e := \{E_1:=\text{span}(e_1), ...,E_n:=\text{span}(e_n)\}$. Consider the action of $U(n)$ on $F_n$ defined by multiplication $$g\cdot \{W_1, ..., W_n\} := \{g W_1, ..., g W_n\}.$$ Let $\{W_1, ..., W_n\}, \{V_1, ..., V_n\}\in F_n$ and choose basis elements of $w_i$ and $v_i$ for each $W_i$ and $V_i$ respectively so that $\{w_i\}_{i=1}^n$ and $\{v_i\}_{i=1}^n$ are orthonormal basis of $\C^n$. Recall from elementary algebra that the transition matrix mapping $\{w_i\}$ onto $\{v_i\}$ is unitary. Therefore this (smooth) action of $U(n)$ on $F_n$ is transitive. Moreover, the isotropy group of $e$ is the torus $T$. So by Theorem \ref{theorem} $$U(n)/T \cong F_n.$$
	Any element $\{W_i\}_{i=1}^n \in F_n$ can be identified with a set of orthogonal projections $\{P_i\}_{i=1}^n$ for $P_i:\C^n\to W_i$.  By orthogonality, $P_iP_j = 0$ if $i\neq j$ and $\sum_{i=1}^n P_i = 1$. Therefore elements of $U(n)/T \times T$ can be identified with pairs $(P, t)$ where $P = (P_1, ..., P_n)$ are orthogonal projections and $t = \text{diag}(p_1(t), ..., p_n(t))$. The $p_i(t)$ can be thought of as the eigenvalues of a unitary matrix $g$, with $P_i$ being the orthogonal projections onto the $p_i(t)$-eigenspace. By requiring $p_1(t)\cdots p_n(t) = 1$, pairs $(P, t)$ can be identified with $\su\times T$.  With this description in mind, the Weyl map $p: SU(n)/T\times T\to SU(n)$ becomes \begin{align} \label{weylmapdescription} (P, t)\mapsto \sum_{i}p_i(t)P_i \end{align} To see this, consider the identification \begin{gather*}
	T\times \su \to T\times F_n\\
	(t, gT) \mapsto (t, gE_1g^{-1}, ..., gE_ng^{-1}).
	\end{gather*} Then $$p(t, gT) = gtg^{-1} = g\left(\textstyle \sum_{i=1}^n p_i(t)E_i\right)g^{-1} =  \textstyle \sum_{i=1}^n p_i(t) \left(gE_ig^{-1}\right)$$ so $p(t, gE_1g^{-1},..., gE_ng^{-1}) =   \textstyle \sum_{i=1}^n t_i \left(gE_ig^{-1}\right)$, giving us the description of the Weyl map on $T\times F_n$ above. 
	\subsection{Connective structure on the cup product bundle gerbe} 
	In this section we aim to compute blah blah blah  in three steps. Herein we shall refer to a bundle gerbes $ \left(J_i \cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i\in \{1, ..., n\}$ as the \textit{$i$-th cup product bundle gerbe}.
	% Recall the line bundle $\widetilde{J}_i\to \su$ with $\widetilde{J}_i := SU(n)\times \C /\sim_{\widetilde{p}_i}$ defined in Example \ref{ex 1}. 
	\begin{proposition}\label{curvaturetwoform}
		For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla^{{J}_i}$ on ${J}_i\to \su$ with curvature $F_{\nabla_{{J}_i}} = \textup{tr}(P_idP_idP_i)$ for $P_i:\su\times \C^n\to J_i $ orthogonal projection which is point-wise a map $P_i(gT): \{gT\} \times \C^n\to (J_i)_{gT} \subset \{gT\}\times \C^n$. 
	\end{proposition}
	
	%\begin{proposition}
	%	For each $i= 1, ..., n$, there is a canonical line bundle connection $\nabla_i$ on $J_i\to T\times \su$ with curvature $$F_{\nabla_i} = \text{tr}(P_idP_idP_i)$$ for $P_i:\su\times \C\to J_i$ orthogonal projection. 
	%\end{proposition}
	\begin{proof} To show this, we will utilise Example \ref{linebundleconnection}. To do so, let us first understand ${J}_i$ as a subbundle of a trivial bundle of rank $n$. Now, ${J}_i$ is a subbundle of the $SU(n)$-homogeneous line bundle $\frac{SU(n)\times \C^n}{T}\to \su$. The latter is isomorphic to the trivial bundle $\su \times \C^n \to \su$ by Theorem \ref{thrmbundles}. Therefore by Example \ref{linebundlecurvature} projection of the trivial connection gives us a connection $\nabla_{{J}_i}:= P_i(d)$ on ${J}_i\to \su$ with curvature two form $F_{\nabla_{{J}_i}} = \text{tr}(P_idP_idP_i)$. \end{proof}
	
	\begin{remark}\label{remark curvatureofJ} 
		Recall that (abusing notation) we have the line bundle $J_i \to T\times \su$ defined by pulling back $J_i\to \su$ along $T\times \su\to \su$. Using that there is an induced pullback connection on $J_i\to T\times \su$, it is not difficult to show by the previous proposition that the pullback connection on $J_i\to T\times \su$ has curvature $\text{tr}(P_idP_idP_i)$ for $P_i: \su \times T\times \C^n \to J_i$ orthogonal projection. Just as we abuse notation with the line bundles $J_i$, we abuse notation and write the curvatures of the connections on these respective line bundles as $\text{tr}(P_idP_idP_i)$ despite the projections being defined on different spaces. 
	\end{remark}
	
	%
	%\begin{corollary}\label{curvatureofJ} 
	%	For each $i=1, ..., n$ there is a canonical line bundle connection $\nabla^{J_i}$ on $J_i\to T\times \su$ with curvature $$F_{\nabla^{J_i}} = \textup{tr}(P_idP_idP_i) $$ for $P_i:T\times \su \times \C \to J_i$ orthogonal projection.
	%\end{corollary}
	%\begin{proof}
	%Recall that $J_i := \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1} \widetilde{J}_i$ for $\pi_{\smath{ \dfrac{SU(n)}{T} } }: T\times \su \to \su$ projection. So we can pullback the connection $\nabla^{\widetilde{J}_i}$ on $\widetilde{J}_i\to \su$ defined above to obtain the connection $$\nabla^{J_i}:= \pi_{\smath{ \dfrac{SU(n)}{T} } }^{-1}\nabla^{\widetilde{J}_i}$$ on $J_i\to T\times \su$. This connection has curvature two form $F_{\nabla^{J_i}} = \pi_{\smath{ \dfrac{SU(n)}{T} } }^{*} F_{\nabla^{\widetilde{J}_i}}$. Pulling back the curvature two form $F_{\nabla^{\widetilde{J}_i}}$ from Proposition \ref{curvaturetwoform} is equivalent to pulling back the orthogonal projections $\su \times \C\to \widetilde{J}_i$ in its definition along $\su\times T \times \C\to \su\times \C$, giving us the result. {\textcolor{red}{is this right?}} 
	%\end{proof}
	
	
	\begin{proposition}\label{existsconnectiononcup} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Let $f:M\to S^1$ be a smooth map. For each $k\in \Z$ define the projection $$\pi_k: \{k\}\times f^{-1}(\R)\to M.$$Then on the cup product bundle gerbe $\left(P\cup f, f^{-1}(\R), M\right)$ there is a bundle gerbe connection $\nabla_{P\cup f}$ with curvature two-form $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ on connected components of $\Z\times f^{-1}(\R) \cong f^{-1}(\R)^{[2]}$.  
	\end{proposition}
	\begin{proof}
		Over $\{k\}\times f^{-1}(\R)$, $P\cup f = \pi_k^{-1}(P)^k$, so $\pi_k^{-1}(\nabla)^k$ defines a connection on connected components $\{k\}\times f^{-1}(\R)$ of $\Z\times f^{-1}(\R)$, hence defines a global connection $\nabla_{P\cup f}$ on $P\cup f \to \Z\times f^{-1}(\R)$. This is a bundle gerbe connection since, for $(n, t_1, t_2, t_3)\in f^{-1}(\R)^{[2]}$ and $m$ the bundle gerbe multiplication on $P\cup f$, $$m\left((P_n)^{t_1-t_3}\otimes (P_n)^{t_1-t_2}\right) = (P_n)^{t_1-t_3}$$ implies $$m(\nabla^{t_1-t_2}\otimes 1 + 1\otimes \nabla^{t_1-t_2}) = \nabla^{t_1-t_3}, $$ which is precisely what it means for $\nabla_{P\cup f}$ to be a bundle gerbe connection in this instance. It then follows immediately by Proposition \ref{constructingconnections} that $$F_{\nabla_{P\cup f}} \big |_{\{k\}\times f^{-1}(\R)} = k\cdot \pi_k^{*}F_{\nabla}$$ for all $k\in \Z$.
	\end{proof}
	\begin{example}\label{connectiononJ}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ for $i= 1, ..., n$. For each $k\in \Z$ let $$\pi_{k,i}: \{k\}\times p_i^{-1}(\R)\to T\times \su $$ be projection and $\nabla_{J_i}$ a connection on $J_i\to T\times \su$. Then by the previous proposition, there is a bundle gerbe connection $\nabla_{J_i\cup p_i}$ on the $i$-th cup product bundle gerbe with two-curvature $$ F_{\nabla_{J_i\cup p_i}}\big |_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_{k,i}^{*}F_{\nabla_{J_i}}.$$
	\end{example}
	
	
	%\begin{proposition}\label{connectiononJ}
	%Consider the $i$-th cup product bundle gerbe for $i\in \{1, ..., n\}$.  Let $k\in \Z$, and define the projection $$\pi_{k}: \{k\}\times p_i^{-1}(\R) \to \su $$ onto the $\su$ element of $p_i^{-1}(\R)$. There is a bundle gerbe connection $\nabla^{\cup_i}$ on the $i$-th cup product bundle gerbe with curvature two-form $$F_{\nabla^{\cup_i}} \big\rvert_{\{k\}\times p_i^{-1}(\R)} = k\cdot \pi_k^{-1}\left(F_{\nabla^{\widetilde{J}_i}}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)\cong p_i^{-1}(\R)^{[2]}$.
	%\end{proposition}
	%
	%\begin{proof} Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ as in Remark \ref{isocup}. To define a line bundle connection on $J_i\cup p_i\to \Z\times \left(\widetilde{p}_i\right)^{-1}(\R) \times \su$ it suffices to define a connection on connected components $U_k:= \{k\}\times p_i^{-1}(\R)$ for $k\in \Z$. Recall $\widetilde{J}_i\to \su$ has line bundle connection $\nabla^{\widetilde{J}_i}$. Hence $\nabla^{\widetilde{J}_i^k}$ is a connection on $\widetilde{J_i}^k \to \su$. So $\pi_k^{-1}\nabla^{\widetilde{J}_i}$ defines a connection on $\pi_k^{-1}\widetilde{J}_i^k \cong J_i\cup p_i \big\rvert_{\{k\}\times p_i^{-1}(\R)}$ This is a bundle gerbe connection because $\nabla^{\widetilde{J}_i}$ is. It follows immediately that the two curvature of the connection $\pi_k^{-1}\left(\nabla^{\widetilde{J}_i^k}\right)$ is $k\cdot \pi_k^{-1}(F_{\nabla^{\widetilde{J}_i}})$ by Proposition \ref{constructingconnections}. \end{proof}
	\begin{remark}
		By Proposition \ref{tensorproductconnection} and Proposition \ref{constructingconnections}, there is a bundle gerbe connection $\nabla^{\otimes \cup}$ on  $ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$ with curvature two form $$F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{*}\left(F_{\nabla^{{J}_i}}\right)  $$ over connected sets $\{(k_1, ..., k_{n-1})\}\times \R^{n-1}\times \su \subset \Z^{n-1}\times \R^{n-1}\times \su \cong \left(\R^{n-1}\times \su\right)^{[2]}$ with $k_n := -k_1 - \cdots - k_{n-1}$. By Remark \ref{remark curvatureofJ} this can be written as $$ F_{\nabla^{\otimes \cup}} = \sum_{i=1}^n k_i\cdot \pi_{k_i,i}^{-1}\left(\text{tr}(P_idP_idP_i)\right)$$ for $P_i: T\times \su \times \C^n \to {J}_i$ orthogonal projection. 
	\end{remark}
	%\text{}\\ 
	%of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$
	
	
	
	
	
	\begin{proposition} \label{curvaturetheorem1} 
		Let $P\to M$ be a line bundle with connection $\nabla$ and curvature two-form $F_\nabla$. Consider the cup product bundle gerbe $(P\cup f, f^{-1}(\R), M)$ defined for $f:M\to S^1$ a smooth map. Let $\pi:f^{-1}(\R)\to M$ be the surjective submersion in this bundle gerbe and $\nabla_{P\cup f}$ the bundle gerbe connection from Proposition \ref{existsconnectiononcup}. Define a two-form $h$ on $f^{-1}(\R)$ by $$h(m, x) = x \cdot \pi^*F_\nabla. $$ Then 
		\begin{enumerate}[(1),font=\upshape]
			\item the two form $h$ satisfies $\delta(h) = F_{\nabla_{P\cup f}}$, so $h$ is a curving for the bundle gerbe connection $\nabla_{P\cup f}$;
			\item the three-curvature $\mu \in \Omega^3(M)$ of the bundle gerbe connection $\nabla_{P\cup f}$ is given by $$\mu =  \frac{1}{2\pi}\, f^{*}(d\theta) \wedge F_{\nabla} $$ for $\theta \in (0,2\pi)$ the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class of $(P\cup f, f^{-1}(\R), M)$ is 
			$$\frac{-i}{4\pi^2}\, f^{*}(d\theta) \wedge F_{\nabla}.$$ 
		\end{enumerate}
	\end{proposition}
	
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	
	\begin{proof} Let us first compute $\delta(h)$. Now, for $(m, x, x') \in f^{-1}(\R)^{[2]}$
		
		\begin{align*}
		\delta(h)\big\rvert_{(m, x, x')} &= \pi_1^{-1} h \big \rvert_{(m, x, x')}   - \pi_2^{-1}h\big\rvert_{(m, x, x')} \\ 
		&=  h\big\rvert_{(m, x')}\circ d\pi_1-  h\big\rvert_{(m, x)}\circ d\pi_2
		\end{align*}
		By noting that $T\Z = 0$ and $f^{-1}(\R)^{[2]} \cong \Z \times f^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla}\big\rvert_{(m, x')} = \pi^{-1}F_{\nabla}\big\rvert_{(m, x)}$. Therefore at a point $(m, x, x')\in f^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
		\delta(h) &= k \cdot \pi^{-1}F_{\nabla}\circ d\pi_1 \big |_{\{k\}\times f^{-1}(\R)}\\ 
		&= k\cdot (\pi\circ\pi_1 |_{\{k\}\times f^{-1}(\R)})^{-1}F_{\nabla}\\
		&= k\cdot \pi_k^* F_{\nabla}\\
		&= F_{\nabla_{P\cup f}}\big |_{\{k\}\times f^{-1}(\R)}.
		\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu\in \Omega^3\left(M\right)$ is defined implicitly by $$dh = \pi^{*}\mu.$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (f\circ \pi)^{*}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
		dh&= d\left(x \cdot \pi^{*}F_\nabla\right)\\
		&= dx \wedge \pi^{*}F_{\nabla}\\
		&= \frac{1}{2\pi} \, \pi^{*}\left(f^{*}(d\theta)\wedge F_{\nabla}\right). 
		\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	
	\begin{example}
		Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ with surjective submersion $\pi_i: p_i^{-1}(\R)\to T\times \su$  and connection and curvature $\nabla^{\cup_i}$, $F_{\nabla^{\cup_i}}$. By the previous proposition, this bundle gerbe has curving $h_i \in \Omega^2(p_i^{-1}(\R))$ given by $$h_i(t, gT, x) = x\cdot \pi_i^* F_{\nabla^{J_i}}$$ and three-curvature $\mu_i\in \Omega^3(T\times \su)$ given by $$\mu_i = \frac{1}{2\pi}\, p_i^*(d\theta) \wedge F_{\nabla^{J_i}}.$$ Moreover, the Dixmier-Douady class of the $i$-th cup product bundle gerbe is $$-\frac{i}{2\pi^2}\, p_i^*(d\theta)\wedge F_{\nabla^{J_i}}. $$
	\end{example}
	
	
	%
	%
	%\begin{proposition}
	%	%Let $\left(J_i\cup p_i, p_i^{-1}(\R), T\times \su\right)$ be a cup product bundle gerbe  for $i\in \{1, ..., n\}$.
	%	Consider the $i$-th cup product bundle gerbe with surjective submersion $\pi: p_i^{-1}(\R)\to T\times \su$, connection $\nabla^{\cup_i}$ and curvature $F_{\nabla^{\cup_i}}$. Define a two-form on $p_i^{-1}(\R)$ by $$h_i(t, gT, x) =  x \cdot \pi^{-1}\left(F_{{\nabla}^{J_i}}\right).$$ Then \begin{enumerate}[(1),font=\upshape]
	%		\item the two-form $h_i$ satisfies $\delta(h_i) = F_{\nabla^{\cup_i}}$, so $h_i$ is a curving for the bundle gerbe connection $\nabla^{\cup_i}$;
	%		\item the three curvature of the bundle gerbe connection $\nabla^{\cup_i}$ is given by $$\mu_i = \textstyle \frac{1}{2\pi}p_i^{-1}(d\theta) \wedge F_{\nabla^{J_i}} $$ for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
	%		\item the Dixmier-Douady class of the $i$-th cup product bundle gerbe is 
	%		$$\frac{-i}{4\pi^2}p_i^{-1}(d\theta) \wedge F_{\nabla^{\cup_i}}.$$ 
	%	\end{enumerate}
	%	\end{proposition}
	%\begin{proof} Let us first compute $\delta(h_i)$. Now, for $(t, gT, x, x') \in p_i^{-1}(\R)^{[2]}$ \begin{align*}
	%\delta(h_i)\big\rvert_{(t, gT, x, x')} &= \pi_1^{-1} h_i \big \rvert_{(t, gT, x, x')}   - \pi_2^{-1}h_i \big\rvert_{(t, gT, x, x')} \\ 
	%&=  h_i\big\rvert_{(t, gT, x')}\circ d\pi_1-  h_i\big\rvert_{(t, gT, x)}\circ d\pi_2
	%\end{align*}
	%By noting that $T\Z = 0$ and $p_i^{-1}(\R)^{[2]} \cong \Z \times p_i^{-1}(\R)$, we see that $d\pi_1 = d\pi_2$. Also, $\pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x')} = \pi^{-1}F_{\nabla^{J_i}}\big\rvert_{(t, gT, x)}$. Therefore at a point $(t, gT, x, x')\in p_i^{-1}(\R)^{[2]}$ with $k := x'-x$, we find \begin{align*}
	%\delta(h_i) &= k \cdot \pi^{-1}F_{\nabla^{J_i}}\circ d\pi_1\\ 
	%&= k\cdot (\pi\circ\pi_1)^{-1}F_{\nabla^{J_i}}\\
	%&= k\cdot \left(\pi_{\smath{ \dfrac{SU(n)}{T} } }\circ \pi \circ \pi_1\right)^{-1} F_{\nabla^{\widetilde{J}_i}}\\
	%&= k \cdot \pi_k^{-1}F_{\nabla^{\widetilde{J}_i}}\\
	%&= F_{\nabla^{\cup_i}}.
	%\end{align*} This shows $(1)$. To show $(2)$, recall that the three curvature $\mu_i \in \Omega^3\left(T\times \su\right)$ is defined implicitly by $$dh_i = \pi^{-1}(\mu_i).$$ Let $x \in (0,1)$ denote the standard coordinate on $\R$, and note that $dx = (p_i\circ \pi)^{-1}\left(\textstyle \frac{d\theta}{2\pi}\right)$ for $\theta \in (0, 2\pi)$ the standard coordinate on $S^1$. Therefore \begin{align*}
	%dh_i &= d\left(x \cdot \pi^{-1}\left(F_{\nabla^{J_i}}\right)\right)\\
	%&= dx \wedge \pi^{-1}\left(F_{\nabla^{J_i}}\right)\\
	%&= \pi^{-1}\left(\textstyle \frac{1}{2\pi} p_i^{-1}(d\theta)\wedge F_{\nabla^{J_i}}\right). 
	%\end{align*} This gives us the claimed three curvature in $(2)$, and $(3)$ follows immediately. \end{proof}
	% Let us first construct the connection on the cup product bundle gerbe. Consider a connected open subset $U\subseteq f^{-1}(\R)^{[2]}$. Recall that $f^{-1}(\R)^{[2]}$ consists of triples $(m, t_1, t_2) \in M\times \R^2$ satisfying $f(m) = [t_1] = [t_2]$. The difference map $d:\R^{[2]}\to \Z$ is continuous and therefore constant on connected components. Therefore for all $(m, t_1, t_2) \in U$, $t_1-t_2 = k$ for some fixed integer $k$. {\textcolor{red}{need to think about connectedness of product I'm getting confused}} Therefore $$(P\cup f)|_U = P^k|_U.$$ Let $\nabla$ be a connection on $P\to M$. Then $\nabla^k$ is a connection on $(P\cup f)|_{U_k}$. Since we can do this for all connected subsetes $U_k$ of $f^{-1}(\R)^{[2]}$, we have a connection $\nabla^{P\cup f}$ on all of $P\cup f$. To see that this is a bundle gerbe connection, recall that bundle gerbe multiplication on $P\cup f$ is given by $$(P_m)^{t_2-t_3} \otimes (P_m)^{t_1-t_2} = (P_m)^{t_1-t_3}.$$ Certainly $$\nabla^{t_1-t_2}\otimes \nabla^{t_1-t_2} = \nabla^{t_1-t_3}$$ so this connection respects the bundle gerbe multiplication.\text{}\\ \text{}\\ 
	%\indent Let $\{U_\alpha\}_{\alpha \in I}$ be an open cover of $M$ such that for each $U_\alpha$ there exists a non-vanishing section $s_\alpha: U_\alpha\to P$. Then there exists connection one forms $A_\alpha \in \Omega^1(U_\alpha)$ for which the connection $\nabla$ on $P\to M$ satisfies $$\nabla s_\alpha = A_\alpha s_\alpha.$$ Let us now find an expression for the connection one forms on $P\cup f\to f^{-1}(\R)^{[2]}$. It suffices to find the connection one forms corresponding to the connection $\nabla^k$ on $P^k|_{U_k}\to {U_k}$ by the above discussion. It is easy to verify that on $P^k|_{U_k}\to {U_k}$ the connection one forms are $$kA_\alpha \in \Omega^1(U_k\cap U_\alpha).$$ Therefore locally $F_{\nabla^k} = kdA_\alpha$, and since $F_{\nabla^{P\cup f}|_{U_k}} = F_{\nabla^k}$, this gives us a local expression for $F_{\nabla^{P\cup f}}$. Next, define $f\in \Omega^2(f^{-1}(\R))$ by $f(m, x) = x\cdot \pi^* F_\nabla$ where $\pi:f^{-1}(\R) \to M$ is the projection map. It can be verified that $f$ is a curving for $kA_\alpha$, that is, (locally) $\delta(f) = kdA_\alpha$ (where we are really pulling the latter two form back by the projection $f^{-1}(\R)^{[2]}\to M$). We can now compute the three-curvature. Now,  \begin{align*}
	%df = d(x\pi^*F_\nabla) = dx\wedge \pi^*F_\nabla = \pi^*(f^* d\theta \wedge F_\nabla)
	%\end{align*} 
	%{\textcolor{red}{really confused with this entire thing. struggling to write this concisely without using all of the pullbacks hidden in here. Also don't understand why we have $d\theta$ here when we actually want it to be $\lambda_k^*d\theta$. }}
	\begin{corollary}\label{corollary data on cup prod} 
		Consider the tensor product of the cup product bundle gerbes$$ \left(\Motimes_{i=1}^n J_i \cup p_i, \R^{n-1}\times \tfrac{SU(n)}{T}, T\times \tfrac{SU(n)}{T}\right)$$ with connection $\nabla^{\otimes \cup}$ and curvature $F_{\nabla^{\otimes \cup}}$. Let $h_i$ and $\mu_i$ be the curving and three curvature respectively of the $i$-th cup product bundle gerbe with connection $\nabla^{\cup_i}$. Let $P_i$ be orthogonal projection $T\times \su\times \C^n\to J_i$. Then \begin{enumerate}[(1),font=\upshape]
			\item the two form $$h := \sum_{i=1}^n h_i$$ on $\R^{n-1}\times \su$ satisfies $\delta(h) = F_{\nabla^{\otimes \cup}}$, ie. $h$ is a curving for the connection $\nabla^{\otimes \cup}$;
			\item the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1} dp_i\wedge \textup{tr}(P_idP_idP_i)$$for $\theta \in (0,2\pi)$ is the standard coordinate chart on $S^1$;
			\item the Dixmier-Douady class is $$\frac{-i}{4\pi^2}\sum_{i=1}^n p_i^{-1} d p_i\wedge \textup{tr}(P_idP_idP_i).$$ 
		\end{enumerate}
	\end{corollary}
	\begin{proof}  By Theorem \ref{curvaturetheorem1}, the three curvature of $\nabla^{\otimes \cup}$ is given by $$\mu = \frac{1}{2\pi}\sum_{i=1}^n p_i^{-1}(d\theta)\wedge \text{tr}(P_idP_idP_i)$$ and the Dixmier-Douady class is $\frac{1}{2\pi i } \mu$. Using the coordinates $\theta = -i\log$ on $S^1$, we find that the pullback of $d\theta$ by $p_i: T\times \su \to S^1$ is $$p_i^{-1}(d\theta) = -i\frac{dp_i}{p_i}.$$ Therefore the three curvature of $\nabla^{\otimes \cup}$ can be rewritten as $$\mu = \frac{1}{2\pi i}\sum_{i=1}^n p_i^{-1}dp_i \text{tr}(P_idP_idP_i),$$ and similarly for the Dixmier-Douady class.\end{proof}
	
	%I am proving the following proposition. 
	%\begin{proposition}\label{connectiononJ}
	%	Consider the $i$-th cup product bundle gerbe $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ for each $i=1, ..., n$. Identify $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$ and denote the surjective submersion $\Z\times p_i^{-1}(\R)\to T\times \su$ by $\pi$. Then for each $i=1, ..., n$, there is a bundle gerbe connection $\nabla^{J_i\cup p_i}$ on $\left(J_i\cup p_i, p^{-1}(\R), T\times \su\right)$ with curvature two-form given by $$F_{\nabla^{J^i\cup p_i}} \big\rvert_{\{n\}\times p_i^{-1}(\R)} = n \cdot \pi^{-1}\left(F_{\nabla_i}\right)$$ on connected components of $\Z\times p_i^{-1}(\R)$.
	%\end{proposition}
	
	%	\textit{Proof}. Consider a connected component $U_n:= \{n\}\times p_i^{-1}(\R)$ of $p_i^{-1}(\R)^{[2]}\cong \Z\times p_i^{-1}(\R)$. Then $J_i\cup p_i \big\rvert_{U_n}= J_i^n$. Note that the pull back of the line bundle $J_i^n \to T\times \su$ by $\pi\rvert_{{U_n}}$ is equal to $(J_u\cup p_i)\big\rvert_{U_n} \to U_n$ defined in the cup product bundle gerbe construction. The line bundle $J_i^n\to T\times \su$ has connection $\nabla_i^n$ by Propositions \ref{connectiononJ} and \ref{tensorproductconnection}. So over connected components $\{U_n\}_{n\in \Z}$ of $p_i^{-1}(\R)^{[2]}$, we can define a connection on $J_i\cup p_i$ by  $$\nabla^{J_i\cup p_i}\big\rvert_{U_n} = \pi^{-1}\left(\nabla_i^n\right). $$ Recall from Proposition \ref{constructingconnections}, the curvature two-form of $\nabla_i^n$ is $$F_{\nabla_i^n} = n \cdot F_{\nabla_i}. $$ Therefore for each $n\in \Z$, the curvature two-form of $\nabla^{J_i\cup p_i}\big\rvert_{U_n}$ is $$F_{\nabla^{J_i\cup p_i}}\big\rvert_{U_n} =n \cdot \pi^{-1}\left(F_{\nabla_i}\right).$$
	
